Extreme-Value Theorems for Optimal Multidimensional Pricing

We provide a near-optimal, computationally efficient algorithm for the unit-demand pricing problem, where a seller wants to price n items to optimize revenue against a unit-demand buyer whose values for the items are independently drawn from known distributions. For any chosen accuracy eps>0 and item values bounded in [0,1], our algorithm achieves revenue that is optimal up to an additive error of at most eps, in polynomial time. For values sampled from Monotone Hazard Rate (MHR) distributions, we achieve a (1-eps)-fraction of the optimal revenue in polynomial time, while for values sampled from regular distributions the same revenue guarantees are achieved in quasi-polynomial time. Our algorithm for bounded distributions applies probabilistic techniques to understand the statistical properties of revenue distributions, obtaining a reduction in the search space of the algorithm via dynamic programming. Adapting this approach to MHR and regular distributions requires the proof of novel extreme value theorems for such distributions. As a byproduct, our techniques establish structural properties of approximately-optimal and near-optimal solutions. We show that, for values independently distributed according to MHR distributions, pricing all items at the same price achieves a constant fraction of the optimal revenue. Moreover, for all eps >0, g(1/eps) distinct prices suffice to obtain a (1-eps)-fraction of the optimal revenue, where g(1/eps) is quadratic in 1/eps and independent of n. Similarly, for all eps>0 and n>0, at most g(1/(eps log n)) distinct prices suffice if the values are independently distributed according to regular distributions, where g() is a polynomial function. Finally, when the values are i.i.d. from some MHR distribution, we show that, if n is a sufficiently large function of 1/eps, a single price suffices to achieve a (1-eps)-fraction of the optimal revenue.

==> bibliography.tex <==
\begin{thebibliography}{1}
%
%\bibitem{BH} X. Bei, Z. Huang. Towards Optimal Bayesian Algorithmic Mechanism Design. {\em SODA} 2011, to appear.          
%
%\bibitem{BGGM} S.~Bhattacharya, G.~Goel, S.~Gollapudi and K.~Munagala. Budget constrained auctions with heterogeneous items. {\em Proceedings of the ACM Symposium on Theory of Computing, STOC} 2010.

%\bibitem{BH} L.~Blumrosen and T.~Holenstein. Posted prices vs. negotiations: an asymptotic analysis. {\em Proceedings of the ACM Conference on Electronic Commerce, EC} 2008.

%\bibitem{BCKW} P.~Briest, S.~Chawla, R.~Kleinberg and S.~M.~Weinberg. Pricing Randomized Allocations. {\em Proceedings of SODA} 2010.

%\bibitem{BK} P.~Briest. Uniform Budgets and the Envy-Free Pricing Problem. {\em Proceedings of ICALP} 2008.

%\bibitem{CDW} Y.~Cai, C.~Daskalakis and S.~M.~Weinberg. An Algorithmic Characterization of Multi-Dimensional Mechanisms. {\em Proceedings of the ACM Symposium on Theory of Computing, STOC} 2012.

%\bibitem{CHK} S.~Chawla, J.~D.~Hartline and R.~D.~Kleinberg. Algorithmic Pricing via Virtual Valuations. {\em Proceedings of the ACM Conference on Electronic Commerce,} EC 2007.
%
%\bibitem{CHMS} S.~Chawla, J.~D.~Hartline, D.~Malec and B.~Sivan. Multi-Parameter Mechanism Design and Sequential Posted Pricing. {\em Proceedings of the ACM Symposium on Theory of Computing, STOC} 2010.

%\bibitem{CMS} S.~Chawla, D.~Malec and B.~Sivan. The Power of Randomness in Bayesian Optimal Mechanism Design. {\em Proceedings of the ACM Conference on Electronic Commerce, EC}, 2010.

%\bibitem{DP} C.~Daskalakis and G.~Pierrakos. Simple, Optimal and Efficient Auctions. {\em Proceedings of the Workshop on Internet \& Network Economics, WINE} 2011.


%\bibitem{DW} C.~Daskalakis and S.~M.~Weinberg. On Optimal Multi-Dimensional Mechanism Design. {\em arXiv,} 2011.

%\bibitem{DR} S.~Dughmi and T.~Roughgarden. Black-Box Randomized Reductions in Algorithmic Mechanism Design. {\em FOCS} 2010.

%\bibitem{extreme} L.~de Haan and A.~Ferreira. {\em Extreme Value Theory: An Introduction}. Springer Series in Operations Research, 2006.

%\bibitem{durrett2} R.~Durrett. {\em Random Graph Dynamics}. Cambridge University Press, 2006.


%\bibitem{HKM} J. Hartline, R. Kleinberg, A. Malekian. Multi-Parameter Bayesian Algorithmic Mechanism Design. {\em SODA} 2011, to appear.

%\bibitem{HL} J.~D.~Hartline and B.~Lucier. Bayesian Algorithmic Mechanism Design. {\em STOC} 2010.

%\bibitem{HK} J.~D.~Hartline and V.~Koltun. Near-Optimal Pricing in Near-Linear Time. {\em Proceedings of WADS,} 2005.

%\bibitem{MV2} A.~M.~Manelli and D.~R.~Vincent. Bundling as an Optimal Selling Mechanism for a Multiple-Good Monopolist. {\em Journal of Economic Theory,} 127(1):1--35, 2006.

%\bibitem{optimal:econ}  A.~M.~Manelli and D.~R.~Vincent. Multidimensional Mechanism Design: Revenue Maximization and the Multiple-Good Monopoly. {\em Journal of Economic Theory,} 137(1):153--185, 2007. 
%
%\bibitem{myerson} R.~B.~Myerson. Optimal Auction Design. {\em Mathematics of Operations Research,} 1981.

%\bibitem{AGTbook} N.~Nisan, T.~Roughgarden, E.~Tardos and V.~V.~Vazirani (eds.). {\em Algorithmic Game Theory}. Cambridge University Press, 2007.

%\bibitem{PV} M.~Pai and R.~Vohra. Optimal auctions with financially constrained bidders. {\em Working Paper,} 2008.

%\bibitem{Than} J.~Thanassoulis. Haggling over substitutes. {\em Journal of Economic Theory,} 117(2):217Ð245, 2004.

%\bibitem{Wil} R.~B.~Wilson. {\em Nonlinear Pricing.} Oxford University Press, 1997.


\end{thebibliography}

==> blurb.tex <==


\section{Blurbs}

In particular, Section~\ref{sec:smoothness properties} shows that there is a way to discretize the set of candidate prices, as well as the support of the value distributions into finite sets of cardinality {\color{red}$O({\log r\over \epsilon^2})$}, without losing more than an $\epsilon$ fraction of the revenue. The discretization of the prices 

(In particular, notice that Theorem~\ref{lem:reduction} implies that the MHR case can be reduced to this case with $r=r(1/\epsilon)$, where $\epsilon$ is the fraction of the revenue lost in the reduction.)

{\color{red}When $r$ is a constant, that is $r$ is independent of $n$, we develop a  Polynomial-Time Approximation Scheme. Given that the case of MHR value distributions reduces to the this case (Theorem~\ref{lem:reduction}), we also obtain a PTAS for the MHR case. (I use $r$ instead of $c$ to be the ratio between $u_{max}$ and $u_{min}$, since it is no longer a constant....)}

{\color{red} Subsequently, in Section~\ref{sec: cover view of the problem} we lay the conceptual foundations of our algorithm. We describe an indirect way to state our problem in terms of approximating a set of revenue distributions, and discuss the probabilistic approximation theorems that would result in an efficient approximation algorithm. Then in Section~\ref{sec:ptas for discretized problem} we implement the plan outlined in Section~\ref{sec: cover view of the problem}. The skeleton of the algorithm is a dynamic program, whose steps are interleaved with probabilistic approximations that are employed to prune the search space as the algorithm evolves. That the loss due to pruning the search space is not significant follows from a double application of the coupling lemma and the optimal coupling theorem (see, e.g.,~\cite{durrett2}). Finally, in Section~\ref{sec:overall ptas} we put everything together to obtain our main result of this section.}


In the independent case, it is assumed that the buyer's values are drawn independently from these distributions. In the correlated case, we allow correlations in these values. In both cases, we may know the distribution of the values explicitly, or we may have oracle access to the distribution. (In the latter case, the oracle returns the value of the cumulative distribution function at a desired point to within a desired precision in time polynomial in the description of the point and the precision.) 

In view of the apparent hardness, it is natural to look at the approximation problem. 

Computer Scientists have also looked at the problem, with an eye on the efficiency of the designed mechanisms. Naturally, the results  here results here are sparser. Papers~\cite{CHK,CHMS, BGGM} and their references provide background on the algorithmic work on this problem. In~\cite{CHMS}, the authors provide efficient sequential posted price mechanisms achieving constant factor approximations to the optimal revenue in multi-unit auction problems, and generalizations to matroid feasibility constraints. Similarly,~\cite{BGGM} provides constant factor approximations for multi-dimensional settings, where the buyers have additional budget constraints.

Our goal in this paper is to make progress on the pricing prob.


Here is an example claim:  ``If our distributions are supported on a discrete set, then we can also assume that the optimal price vector is supported on the same discrete set.'' This statement is false; see Appendix~\ref{sec:counter}.
%
%For example, the following  smoothness properties that we would like to use turn out to be false:
%\begin{itemize}
%\item ``If we modify a single distribution $F_i$ to a different one $\hat{F}_i$ that is within $\epsilon$ in total variation distance, the optimal revenue in the new instance is within a factor of $(1+g(1/\epsilon))$ from the optimal revenue in the original instance, where $g(\cdot)$ is some decreasing function that does not depend on $n$.'' This statement is false; see Appendix~\ref{sec:counter} for an easy example.
%
%\item ``If our distributions are supported on a discrete set, then we can also assume that the optimal price vector is supported on the same discrete set.'' This statement is also false; see Appendix~\ref{sec:counter}.
%
%\end{itemize}
Given that this and other related smoothness properties are false, we find it extremely hard to discretize the distributions into a constant number of distinct distributions. We can obtain a delicate discretization of the support of the distributions into a bounded set (Lemma~\ref{lem:horizontal-discretization}), but we cannot discretize the probabilities that these distributions use into a bounded set of different probability-values, arriving at an impasse with our discretization idea.


==> figures.tex <==
\section{Figures} \label{sec:figures}
\text{~}
\begin{figure}[h!]
  \centering
  \includegraphics[height = 1.4in]{circuit}\\
   \caption{The Revenue Distribution.}\label{fig:d1}
\end{figure}

==> iid2.tex <==
\section{A Single Price Suffices for I.I.D. MHR Distributions} \label{sec:MHR iid}

%In this section, we will present a generic PTAS for finding the optimal pricing when the distributions are i.i.d. and satisfy MHR. Let $X_1,X_2,\ldots,X_n$ be $n$ i.i.d random variables, which satisfy MHR. We will use $F(x)$ and $f(x)$ to be the cumulative and density function for this distribution. We define a new random variable $M = \max_{i\in[n]} X_i$. 
We provide a faster algorithm for the case where the buyer's values are independent and identically distributed according to some MHR distribution. The main technical idea that goes into the algorithm is this: if the number of items is a sufficiently large function of $\epsilon$, then using a single price suffices to get an $\epsilon$ fraction of the optimal revenue. We proceed to the details of our algorithm. To simplify our notation, let us assume that all the $v_i$'s are independent copies of the random variable $v$, and denote the distribution of $v$ by $F$. Moreover, let $\alpha_n = \inf\left\{x|F(x)\geq 1-\frac{1}{n}\right\}$ (as in Definition~\ref{def:alpha}). We start by showing an analogue of Lemma~\ref{lem:tinycontribution}.
\begin{lemma}\label{lem:iidsmallcontribution}
    If $S=Con[v\geq (1+\epsilon)\alpha_{n}]$, then $S\leq \frac{6(1+\epsilon)\alpha_n}{n^{1+\epsilon}}.$
\end{lemma}

Using Lemma~\ref{lem:iidsmallcontribution} and Lemma~\ref{lem:trunchigh}, we deduce that if we constrain our prices to be $\le (1+\epsilon)\alpha_{n}$, we lose no more most $\frac{6(1+\epsilon)\alpha_n}{n^{\epsilon}}$ revenue. Given that the optimal revenue with the restriction that all prices be $\le (1+\epsilon)\alpha_{n}$ is at most $(1+\epsilon)\alpha_{n}$, it follows that the optimal revenue without the restriction is at most $(1+\epsilon)\alpha_{n}+\frac{6(1+\epsilon)\alpha_n}{n^{\epsilon}} = (1+\epsilon)(1+\frac{6}{n^{\epsilon}})\alpha_n$. This is very close to $\alpha_n$ if $n$ is a sufficiently large function of $\epsilon$. If that's the case, it suffices to find a price vector achieving revenue close to $\alpha_n$.

\begin{lemma}\label{lem:iidalmostopt}
    If we use the price vector $P=((1-\epsilon)\alpha_n,(1-\epsilon)\alpha_n,\ldots,(1-\epsilon)\alpha_n)$, we receive revenue at least $ \left(1-e^{(-n^{\epsilon})}-\epsilon\right)\alpha_{n}$.
\end{lemma}

Notice that, when $n\geq (1/\epsilon)^{1/\epsilon}$, $n^{\epsilon}\geq 1/\epsilon$. In this case, we have shown that $OPT\leq (1+\epsilon)(1+6\epsilon)\alpha_{n}\leq(1+8\epsilon)\alpha_{n}$. On the other hand, Lemma~\ref{lem:iidalmostopt}, says that we can achieve revenue at least $(1-\frac{1}{e^{1/\epsilon}}-\epsilon)\alpha_{n}$ using a single price. Since $e^{1/\epsilon}\geq 1/\epsilon$, this revenue is at least $(1-2\epsilon)\alpha_{n}$. Given that $(1+8\epsilon)(1-10\epsilon)\leq (1-2\epsilon)$, we have $(1-2\epsilon)\alpha_{n}\geq (1-10\epsilon)OPT$. So if we set the price for every item to be $(1-\epsilon)\alpha_{n}$, we achieve a revenue that is at least $(1-10\epsilon)OPT$.
%Let $\rm OPT$ be the expected revenue for the optimal pricing. The following lemma shows that $\rm OPT$ can not be much smaller than $\alpha_n$.

%\begin{lemma}\label{lem:constantfactor}
%    $\rm OPT$$\geq (1-1/e)\alpha_n$ 
%\end{lemma}
%\begin{proof}
%    Consider the following simple pricing scheme, for every item we use the same price $\alpha_n$. The seller will sell an item iff the buyer's value for any item is above $\alpha_n$. So the probability that the seller will sell an item is $1-(1-1/n)^n \geq 1-1/e$. Under this price, the revenue is at least $(1-1/e)\alpha_n$. Thus, $\rm OPT$$\geq (1-1/e)\alpha_n$.
%\end{proof}

%\begin{corollary}
%    $\mathbb{E}[M|M\geq \alpha_{n^2}]\cdot \Pr\{M\geq \alpha_{n^2}\}\leq \frac{4}{n(1-1/e)}OPT$
%\end{corollary}

%By Lemma~\ref{lem:tinycontribution}, we know that the contribution from values above $\alpha_{n^2}$ to expectation is small. The following lemma essentially shows that, the contribution to revenue from prices above $\alpha_{n^2}$ is also small. In fact, we show that for any pricing, we can simply raise the prices which are above $\alpha_{n^2}$ to $+\infty$, of course, the seller extracts $0$ revenue from these prices, but the total revenue only decreases a tiny amount.
 
%\begin{lemma}%\label{lem:trunchigh}
 %   Let $p$ be a pricing, we define $p'$ as follows, if $p_i<\alpha_{n^2}$, $p'_i = p_i$, otherwise $p'_i = 2u_{max}$. $ \mathcal{R}_{p'} > \mathcal{R}_{p}-12\alpha_{n}/n$.
%\end{lemma}
%\begin{proof}
%   Let $\pi_i = \Pr\{\forall j, v_i-p_i\geq v_j-p_j \land v_i-p_i\geq 0 \}$, $\pi'_i = \Pr\{\forall j, v_i-p'_i\geq v_j-p'_j \land v_i-p'_i\geq 0 \}$.
    
%    We define two sets of items based on $p$, $S_{exp} = \{i:p_i > \alpha_{n^2}\}$ and $S_{chp} = \{i:p_i \leq \alpha_{n^2}\}$. If $i\in S_{exp}$, $p'_i = 2u_{max}$, if $i\in S_{chp}$, $p'_i = p_i$.
    
%     For any $i\in S_{exp}$, $\pi_i\geq \pi'_i = 0$. For any $i\in S_{chp}$, $\pi_{i}\leq \pi'_{i}$. Because for any valuation vector $(v_1,v_2,\ldots,v_n)$, if for any $j$, $v_i-p_i\geq v_j-p_j$ and $v_i-p_i\geq 0$, it should also be true that for any $j$, $v_i-p'_i\geq v_j-p'_j$ and $v_i-p'_i\geq 0$ (we only increase the price for some items different from $i$). Therefore, the following inequality holds:
%    $$\sum_{i\in S_{chp}}p_i\cdot \pi_i\leq \sum_{i\in S_{chp}}p'_i\cdot \pi'_i \quad (1)$$
    
%     For any valuation vector $(v_1,v_2,\ldots,v_n)$, we define $v_{max} = \max_{i} v_i$. For any $i\in S_{exp}$, whenever the condition $C_i = \forall j, v_i-p_i\geq v_j-p_j \land v_i-p_i\geq 0$ is true, $p_i$ is smaller than $v_i$ and is smaller than $v_{max}$. Notice that for any of the conditions to be true, it must be that $M\geq \alpha_{n^2}$ is true. On the other hand, for different $i,j \in S_{exp}$, $C_i$ and $C_j$ can not be true simultaneously. So we can upper bound $\sum_{i\in S_{exp}}p_i\cdot \pi_i$ by the expectation of $v_{max}$ in the region that $v_{max}\geq \alpha_{n^2}$, which is exactly $\mathbb{E}[M|M\geq \alpha_{n^2}]\cdot \Pr\{M\geq \alpha_{n^2}\}$. By Lemma~\ref{lem:tinycontribution}, we know that $\mathbb{E}[M|M\geq \alpha_{n^2}]\cdot \Pr\{M\geq \alpha_{n^2}\}$ is no greater than $12\alpha_{n}/n$. 
     
%     Now it is easily seen that the followings are true:
%     $$\mathcal{R}_{p'} \geq \sum_{i\in S_{chp}}p'_i\cdot \pi'_i$$
%     $$\mathcal{R}_{p} = \sum_{i\in S_{chp}}p_i\cdot \pi_i+ \sum_{i\in S_{exp}}p_i \leq \sum_{i\in S_{chp}}p_i\cdot \pi_i+12\alpha_{n}/n$$
     
%     Combining $(1)$, we can show $$\mathcal{R}_{p'} > \mathcal{R}_{p}-12\alpha_{n}/n.$$
     %if the buyer buys an item $i_j$ for any $j\in[k]$, that means $v_{max} = \max_i v_i\geq \alpha_{n^2}$. And notice that $p_{i_j}\leq v_{max}$. The revenue collected from prices that are above $\alpha_{n^2}$ is exactly the expectation of $p_{i_j}$, which is bounded above by the expectation of $v_{max}$. And the expectation of $v_{max}$ is exactly $\mathbb{E}[M|M\geq \alpha_{n^2}]\cdot \Pr\{M\geq \alpha_{n^2}\}$. Thus, the revenue collected from prices that are above $\alpha_{n^2}$ is smaller than $\mathbb{E}[M|M\geq \alpha_{n^2}]\cdot \Pr\{M\geq \alpha_{n^2}\}$, which is smaller than $4\alpha_{n}/n$.
%\end{proof}

%Combining Lemma~\ref{lem:constantfactor} and~\ref{lem:trunchigh}, we know that if $p$ is the optimal pricing, we can ignore the prices that are higher than $\alpha_{n^2}$, and only lose an tiny fraction of the revenue. This gives us an upper bound. If we want to approximate the optimal, we can only consider the prices that are no greater than $\alpha_{n^2}$. The next lemma gives us a lower bound. It essentially demonstrates that we can also throw away the prices that are smaller than $\epsilon\alpha_n$, and only lose a small amount of revenue.
  
 %\begin{corollary}\label{cor:almostopt}
 %    If $p^*$ is the optimal pricing, $\mathcal{R}_{p^*} = \rm OPT$,  we define $\hat{p}$ as follows, if $p^*_i>\alpha_{n^2}$, $\hat{p}_i= 2u_{max}$, if $\epsilon \alpha_n\leq p^*_i\leq \alpha_{n^2}$, $\hat{p}_i = p^*_i$, if $p^*_i<\epsilon\alpha_n$, $\hat{p}_i = \epsilon\alpha_n$. Then $\mathcal{R}_{\hat{p}}\geq \Big(1-\frac{4/n+\epsilon}{(1-1/e)}\Big)\rm OPT$.
 %\end{corollary}
 %\begin{proof}
 %    From Lemma~\ref{lem:trunchigh} and~\ref{lem:trunclow}, we know that the lost on revenue is at most $(4/n+\epsilon)\alpha_n$ by pricing $\hat{p}$. By Lemma~\ref{lem:constantfactor}, we know $\rm OPT\geq(1-1/e)\alpha_n$. So we have $\mathcal{R}_{\hat{p}}\geq \Big(1-\frac{4/n+\epsilon}{(1-1/e)}\Big)\rm OPT$.
 %\end{proof}
 
%\begin{lemma}\label{lem:smallregionsuffice}
%    There exists a pricing $p^{\star}$, for all $i$, $p^{\star}_i\in [\epsilon\alpha_n, 2\alpha_n]$, and $\mathcal{R}_{p^{\star}}\geq \Big(1-\frac{4/n+\epsilon}{(1-1/e)}\Big)\rm OPT$
%\end{lemma}
%\begin{proof}
%    Take $\hat{p}$ in Corollary~\ref{cor:almostopt}, then apply the surgery in Lemma~\ref{lem:decreaseprice} to $\hat{p}$. After the changes, we get a pricing, whose prices are all between $\epsilon\alpha_n$ and $\alpha_{n^2}$, which is smaller than $2\alpha_n$. This is $p^{\star}$. Combining Corollary~\ref{cor:almostopt} and Lemma~\ref{lem:decreaseprice}, we demonstrate that the following inequality is true:
%     $$\mathcal{R}_{p^{\star}}\geq \mathcal{R}_{\hat{p}}\geq \Big(1-\frac{4/n+\epsilon}{(1-1/e)}\Big)\rm OPT$$ 
%\end{proof}
%\begin{lemma}\label{lem:undermax}
 %    Let $p$ be a pricing, $S_{over}= \{i: p_i>u_{max}\}$, $p_{fmax} = max_{i\in[n]/S_{h}}$. We define $p'$ to be the following pricing: $p'_i = p_{fmax}$, for all $i\in S_{over}$, $p'_i=p_i$ otherwise. We have $\mathcal{R}_{p'}\geq\mathcal{R}_{p}$.
 %\end{lemma}
 
 %\begin{proof}
 %    For any valuation vector $(v_1,v_2,\ldots,v_n)$, if $i$ is the winner, that is for any $j$, $v_i-p_i\geq v_j-p_j$ and $v_i-p_i\geq 0$. Then under $p'$, there are two possibilities. (1) $i$ is still the winner, the contribution for revenue is the same under $p$ and $p'$ (2) $i$ is not the winner, but the winner can only be those items that have lower prices than in $p$. So the winner must belongs to set $S_{h}$. For any $j\in S_{h}$, $p'_j = p_{fmax}\geq p_i$, since to be a winner, $p_i$ must be smaller than $u_{max}$. Then the contribution to revenue under $p'$ is higher than under $p$. Thus, $\mathcal{R}_{p'}\geq\mathcal{R}_{p}$. 
%\end{proof}

%\begin{lemma}\label{lem:abovemin}
%    Let $P$ be a price vector, $S_{l}= \{i: p_i<u_{min}\}$. We define $P'$ to be the following price vector: $p'_i = u_{min}$, for all $i\in S_{l}$, $p'_i=p_i$ otherwise. We have $\mathcal{R}_{P'}\geq\mathcal{R}_{P}$.
%\end{lemma}
%\begin{proof}
 %   If $i$ is the winner under $P$ and $i\notin S_{l}$, then $i$ is still the winner under $P'$, since we only increase the prices for some items different from $i$. If $i$ is the winner under $P$ and $i\in S_{l}$, there are two possibilities. (1) $i$ is still the winner, but the contribution now is $u_{min}\geq p_i$. (2)$i$ is not the winner, then there must still be a winner since $v_i-p'_i\geq0$. Then the contribution is still at least $u_{min}\geq p_i$. Thus,  $\mathcal{R}_{P'}\geq\mathcal{R}_{P}$.
%\end{proof}

%\begin{lemma}[Nisan]\label{lem:nisan-price}
%    For any $epsilon\in(0,1)$, let $P$, $P'$ and $P''$ be price vectors that satisfy, for all $i$ $p'_i=(1+\epsilon^2-\epsilon)p''_i$ and $p''_i\in[1-\epsilon^2,1]p_i$. Then $\mathcal{R}_{P'}\geq(1-2\epsilon)R_P$.
%\end{lemma}
\begin{theorem}\label{thm:alg}
If the values of the buyer are i.i.d. according to a MHR distribution, there is a PTAS for finding a price vector that achieves a $(1-\epsilon)$ fraction of the optimal revenue. The algorithm runs in time polynomial in {\color{red}$2^{O({\log^7 (1/\epsilon)\over\epsilon^{19}})}+O(\log({\log n\over \epsilon}))$} and the size of the input. Moreover, if $n\geq (1/\epsilon)^{1/\epsilon}$, there exists an efficiently computable price such that, if all items are priced at this price, the resulting revenue is at least {\color{red} $(1-\epsilon)OPT$}.
   %If the values of the buyer are i.i.d. according to a MHR distribution, there is a PTAS for finding a price vector that achieves a $(1-\epsilon)$ fraction of the optimal revenue. The algorithm runs in time polynomial in $2^{\log^9 (1/\epsilon)/\epsilon^6}$ and the size of the input. Moreover, if $n\geq (1/\epsilon)^{1/\epsilon}$, there exists an efficiently computable price such that, if all items are priced at this price, the resulting revenue is at least $(1-12\epsilon)OPT$. 
\end{theorem}


==> introduction_yang.tex <==
\section{Introduction} \label{sec:intro}


We study the following {pricing problem}. A seller has $n$ items to sell  to a buyer who is looking to buy a single item. The seller wants to maximize profit from the sale, leveraging stochastic knowledge she has about the buyer to achieve this goal. In particular, we assume that the seller has access to a distribution $\cal F$ from which the values $(v_1,\ldots,v_n)$ of the buyer for the items are drawn. Given this information, the seller wants to compute prices $p_1,\ldots,p_n$ for the items  to maximize her revenue, assuming that the buyer is {\em quasi-linear}---i.e. will buy the item~$i$ maximizing $v_i - p_i$, as long as this difference is positive. That is, the seller's expected revenue from a price vector $P=(p_1,\ldots,p_n)$ is
\begin{align}
{\cal R}_P=\sum_{i=1}^n p_i \cdot \Pr \big[ (i = \arg \max\{v_j - p_j\})~\wedge~(v_i-p_i\ge0)\big], \label{eq:objective}
\end{align}
where we assume that the $\arg \max$ breaks ties in favor of a single item, when there are multiple maximizers. A more sophisticated seller could try to improve her revenue by pricing lotteries over items, that is also price randomized allocations of items~\cite{BriestCKW10}, albeit this may be less natural than item pricing, and we will not study it extensively in this paper.

While our problem  has a simple statement, it exhibits rich behavior depending on the nature of $\cal F$. For example, if $\cal F$ assigns the same value to all the items with probability $1$, i.e. when the buyer always values all items equally, the problem becomes {\em single-dimensional}. In this setting, it is clear that lotteries  do not improve  the revenue and that the optimal price vector can assign the same price to all the items. This observation is a special case of the more general, celebrated result of Myerson~\cite{Myerson81} on optimal mechanism design, i.e. the multi-buyer version of our problem, and generalizations thereof. Myerson's result provides a closed-form solution to the multi-buyer problem in a single sweep that covers many settings, but only works under the same limiting assumption that every buyer is single-dimensional, i.e. receives the same value from all the items. (More generally, every buyer receives the same value from all outcomes of the mechanism that provide her service.)

Following Myerson, a large body of research in both Economics and Engineering has been devoted to extending his result to the {\em multi-dimensional setting}, where the buyers' values come from general distributions.  And, while there has been sporadic progress (see survey~\cite{ManelliV07} and its references), an optimal multi-dimensional mechanism, generalizing Myerson's result, does not seem to be in sight. Indeed, there is not even an optimal solution known for the single-buyer item pricing problem.  Even the ostensibly easier version of that problem, where the values of the buyer for the items are independent and supported on a set of cardinality $2$ is unresolved.\footnote{Incidentally, the problem is trickier than it originally seems, and various intuitive properties that one would expect from the optimal solution fail to hold. See Appendix~\ref{sec:counter} for an interesting example.} Our main contribution in this paper is to develop {near-optimal polynomial-time algorithms for this problem,} when the buyer's values for the items are independent.

%Motivated by the importance of multidimensional mechanism design, and intrigued by the simplicity and apparent difficulty of the multidimensional, unit-demand pricing problem, we devote this paper to its study.  

\subsection{Main Results}

We partition our results into algorithmic and structural. The former provide efficient algorithmic procedures for computing near-optimal price vectors. The latter shed light into the structure of optimal solutions.

\paragraph{Algorithmic Results.} Previous work on the item pricing problem has provided constant factor approximation algorithms. The best known polynomial-time algorithm obtains revenue that is at least $1/2$ of the revenue of the optimal price vector~\cite{ChawlaHK07,ChawlaHMS10}. We discuss these approaches in Section~\ref{sec:related}, also noting that they are limited to constant factor approximations. We are aiming instead for item pricing mechanisms that come arbitrarily close to the optimal revenue, obtaining the following results. Their proofs are overviewed in Sections~\ref{sec: cover view of the problem} through~\ref{sec:regular}, while complete details are provided in the appendix.



%Moreover, if the distributions $\{{\cal F}_i\}_i$ are {\em regular} (this is a commonly studied class of distributions in Economics,) the corresponding price vector can be computed efficiently.








%Our goal in this proposal is to push our boundary of understanding towards efficient approximately optimal mechanisms, whose revenue is within a $(1+\epsilon)$ factor of the optimum for any desired positive constant $\epsilon$. Our main tool to approach this problem will be to use insights from Extreme Value Ttheory in Statistics, as explained below.
%\begin{align*}\noindent \begin{minipage}[h]{16cm}$\bullet$ {\bf Research Question 6:} {\em   In what multi-dimensional mechanism-design settings are there polynomial-time mechanisms achieving $(1-\epsilon)$ fraction of the optimal revenue?}\end{minipage} 
%\end{align*}

% Moreover, when the (identical) marginals of $F$ over the items are {\em regular distributions} the price obtaining the optimal revenue is the maximum of a concave function.


%In this paper, our goal is to make progress on the simplest  multi-dimensional mechanism design setting where there is a single unit-demand bidder who is interested in buying one out of $n$ items. In this case, the mechanism design problem degenerates to a pricing problem, called the {\em multi-dimensional unit-demand pricing problem}. More precisely, our setting is the following. The seller has $n$ items for sale, denoted $1,\ldots,n$, and there is a single buyer who is interested to buy a single out of these $n$ items. Moreover, the seller has prior information about the bidder's value for each item. In particular, the seller can model the value that the buyer has for item $i$ as a random variable $v_i$ drawn from some known distribution $\mathcal{F}_i$. In the independent case, it is assumed that the buyer's values are drawn independently from these distributions. In the correlated case, we allow correlations in these values. In both cases, we may know the distribution of the values explicitly, or we may have oracle access to the distribution. (In the latter case, the oracle returns the value of the cumulative distribution function at a desired point to within a desired precision in time polynomial in the description of the point and the precision.) 
%
%Given the Bayesian information that the seller has about the buyer, the seller needs to compute prices $p_1,\ldots,p_n$ for the items, so as to maximize her revenue. Given that the buyer is going to buy item $i$, if $v_i-p_i \ge 0$ and $i \in \arg \max\{v_j - p_j\}$, the expected revenue of the seller for a price vector $P=(p_1,\ldots,p_n)$ is
%$$\sum_{i=1}^n p_i \cdot \Pr\left[ i = \arg \max\{v_j - p_j\}\right],$$
%where we assume that when the $\arg \max$ contains multiple items the buyer choses one of them in a lexicographic order that has been fixed in advance.






\begin{theorem}[{\bf Main Algorithmic Result:} Additive PTAS for Bounded Distributions]\label{thm:additive ptas}
Suppose that the values of the buyer for $n$ items are independent and normalized to lie in $[0,1]$. Then, for all $\epsilon >0$, {there exists an algorithm that computes a price vector whose revenue is within an additive $\epsilon$ of optimal, and whose running time is polynomial in $n^{{\log^{3} 1/\epsilon\over \epsilon^{4}}}$.}
\end{theorem}

\begin{theorem}[General Algorithm]\label{thm:general algorithm}
Suppose that the values of the buyer for $n$ items are independent and supported on some interval $[u_{min},r \cdot u_{min}]$ for some $u_{min} >0$ and $r \ge 1$. Then, for all $\epsilon >0$, there is an algorithm that computes a price vector whose revenue is at least a $(1-\epsilon)$-fraction of the optimal revenue, and whose running time is polynomial in {$\max\left\{n^{\log^{11} r \cdot  \log \log r}, n^{\log^{3} r \cdot\log {1 \over \epsilon}\over \epsilon^{8}}\right\}$}\notshow{$n^{{\rm poly}({1 \over \epsilon}, \log r)}$}.\footnote{We note that a natural approach for computing approximately optimal price vectors is to discretize the domain of price vectors and show that searching over the discretized domain suffices for approximating the optimal revenue. However, a straightforward application of the discretizations  proposed by Nisan~\cite{ChawlaHK07} and Hartline and Koltun~\cite{HartlineK05} to our problem would result in running time of  $\left({1 \over \epsilon} \log r\right)^{O(n)}$. The purpose of our theorem is to remove the exponential dependence of the running time on the number of items $n$.}
\end{theorem}

\begin{theorem}[Multiplicative PTAS for MHR Distributions]\label{thm:ptas mhr}
There is a Polynomial-Time Approximation Scheme\footnote{A Polynomial-Time Approximation Scheme (PTAS) is a family of algorithms $\{\mathcal{A}_{\epsilon}\}_{\epsilon}$, indexed by the accuracy parameter $\epsilon >0$, such that for every fixed $\epsilon>0$, $\mathcal{A}_{\epsilon}$ runs in time polynomial in the size of its input. See Section~\ref{sec:prelim} for a formal definition.} for computing an optimal price vector, when the values of the buyer are independently drawn from Monotone Hazard Rate distributions.\footnote{Monotone Hazard Rate (MHR)  distributions are a commonly studied class of distributions that contain such familiar distributions as the Uniform, Gaussian and Exponential distributions. See Section~\ref{sec:prelim} for a formal definition.} 

For any accuracy $\epsilon >0$, the algorithm runs in time polynomial {in $n^{{1 \over \epsilon^{7}}}$},  and outputs a price vector whose revenue is at least a $(1-\epsilon)$-fraction of the optimal revenue, where $n$ is the number of items.
\end{theorem}

\begin{theorem}[Multiplicative Quasi-PTAS for Regular Distributions]\label{thm:quasi ptas regular}
There is a Quasi-Polynomial-Time Approximation Scheme\footnote{A Quasi-Polynomial-Time Approximation Scheme (Quasi-PTAS) is a family of algorithms $\{\mathcal{A}_{\epsilon}\}_{\epsilon}$, indexed by the accuracy parameter $\epsilon >0$, such that for every fixed $\epsilon>0$, $\mathcal{A}_{\epsilon}$ runs in time quasi-polynomial in the size of its input. See Section~\ref{sec:prelim} for formal definition.} for computing an optimal price vector, when the values of the buyer are independent and drawn from regular distributions.\footnote{Regular distributions are another widely studied class of distributions that contain MHR distributions. See Section~\ref{sec:prelim} for a formal defintion.} 

For any accuracy $\epsilon >0$, the algorithm runs in time {polynomial in $\max\left\{ n^{\log^{11} {n\over \epsilon} \cdot  \log \log {n\over\epsilon}}, n^{ {\log^3 {n\over\epsilon} \cdot  \log {1\over\epsilon} \over {\epsilon}^{8}}} \right\}$},  and outputs a price vector whose revenue is at least a $(1-\epsilon)$-fraction of the optimal revenue, where $n$ is the number of items.
\end{theorem}

\notshow{\yangnote{In fact, Theorem~\ref{thm:general algorithm} easily implies
Theorem~\ref{thm:additive ptas}. When the values are distributed in $[0,1]$, by ignoring the values that are smaller than $\epsilon$, we face a new pricing problem whose values are distributed in $[\epsilon, 1]$. It is not hard to see that for any price vector, the revenue achieved under these two distributions will differ for at most $\epsilon$. If we use the general algorithm to solve the new pricing problem, the solution will be an additive $O(\epsilon)$ approximation for the original problem.(Yang: Reviewer 1 wants this paragraph. Shall we add a graph to show that we prove our theorems by reducing the problems to the general problem.)} }

\paragraph{Discussion of Algorithmic Results.} Prior to our work there were no optimal algorithms known for multi-dimensional auction problems without special structure. In particular, only constant factor approximation algorithms were known for the item pricing problems addressed by Theorems~\ref{thm:additive ptas} through~\ref{thm:quasi ptas regular}. (For an extensive discussion of related work, we refer the reader to Section~\ref{sec:related}.) Our results are the first to obtain near-optimal solutions for these problems in polynomial time. We view the main contribution of our results not to be the practicality of our algorithms, but establishing that there is no lingering constant in-approximability results for item pricing. In particular, our results show that, for any desired accuracy $\epsilon>0$, there are polynomial-time algorithms that compute $\epsilon$-optimal solutions. Complemented with the {\tt NP}-hardness result for the item pricing problem discussed in Section~\ref{sec:related}, what is left open by our work is obtaining faster near-optimal algorithms.

 \paragraph{Structural Results.} Our algorithms are obtained by studying the distribution of the optimal revenue, as a function of the buyer's values (which are random) and the optimal price vector (which is unknown), as overviewed in Section~\ref{sec:techniques}. As a byproduct of our techniques, we deduce the following structural properties of optimal solutions, whose proofs are given in Appendix~\ref{sec:proofs of structural}. {Theorem~\ref{thm:single price constant factor} states that, when the values are independently distributed according to monotone hazard rate distributions,  then pricing all items at the same price guarantees a constant fraction of the optimal revenue. Theorem~\ref{thm:constant prices suffice} generalizes this to showing that only the desired approximation~$\epsilon$ dictates the number of distinct prices that are necessary to achieve a $(1-\epsilon)$-fraction of the optimal revenue, and {not the number of items or the size of the support of the distributions}, as long as they are monotone hazard rate. Theorem~\ref{thm:logn prices suffice} generalizes this result to a mild dependence on $n$ for regular distributions. 

\begin{theorem}[{\bf Structural 1 (MHR):} Constant Factor Approximation from a Single Price] \label{thm:single price constant factor} If the buyer's values for the items are independently distributed according to MHR distributions, there exists a price $p$ such that pricing all items at $p$ guarantees a constant fraction of the optimal revenue. Price $p$ can be computed efficiently from the value distributions.
\end{theorem}}

\begin{theorem}[{\bf Structural 2 (MHR):}  A Constant Number of Distinct Prices Suffice for Near-Optimal Revenue] \label{thm:constant prices suffice} There exists a quasi-quadratic\footnote{A function $g: \mathbb{R}_+ \longrightarrow \mathbb{R}_+$ is {\em quasi-quadratic} iff it satisfies $g(x)=O(x^2 \log^c x)$, for some absolute constant $c>0$. For the meaning of the $O(\cdot)$ notation please refer to Section~\ref{sec:prelim}.} function $g(\cdot)$ such that, for all $\epsilon>0$ and all $n>0$, $g(1/\epsilon)$ distinct prices suffice to achieve a $(1-\epsilon)$-fraction of the optimal revenue, when the buyer's values for the $n$ items are independently distributed according to MHR distributions. These distinct prices can be computed efficiently from the value distributions.
\end{theorem}
\begin{theorem}[{\bf Structural 3 (Regular):}  A Polylogarithmic Number of Distinct Prices Suffice for Near-Optimal Revenue] \label{thm:logn prices suffice} There exists a polynomial function $g(\cdot)$ such that, for all $\epsilon>0$ and $n>0$, $g(1/\epsilon \cdot \log n)$ distinct prices suffice to achieve a $(1-\epsilon)$-fraction of the optimal revenue, when the buyer's values for the $n$ items are independently distributed according to regular distributions. These  prices can be computed efficiently from the value distributions.
\end{theorem}
%\begin{theorem}[{\bf Structural 3:}  Number of Distinct Prices for General Distributions] \label{thm:logr prices suffice} There exists a (polynomial) function $g(\cdot)$ such that, for all $r>0$ and $\epsilon \in (0,{1 \over \log r})$, $g(1/\epsilon \cdot \log r)$ distinct prices suffice for a $(1+\epsilon)$-approximation to the optimal revenue, when the buyer's values for the $n$ items are independent and supported on a set $[u_{min},r u_{min}] \subset \mathbb{R}_+$.
%\end{theorem}
%, while Theorem~\ref{thm:logr prices suffice} to a mild dependence on the support of the distributions in the general case. 
%A natural approach to show Theorem~\ref{thm:logr prices suffice} would be to use a discretization lemma attributed to Nisan~\cite{CHK}. Unfortunately, the resulting dependence of the number of distinct prices on $r$ is polynomial, so we need to develop a more intricate discretization scheme that is much more stringent. The details of our argument are presented in  Section~\ref{sec:balanced range}. 

Finally, it seems intuitive that, when the value distributions are not widely different, a single price might suffice for extracting a $(1-\epsilon)$-fraction of the optimal revenue, as long as there is a sufficient number of items for sale. We show such a result for the case where the buyer's values are i.i.d. according to a MHR distribution. See Appendix~\ref{sec:MHR iid} for the proof of this theorem.

%an upper bound on the optimal revenue is clearly $\mathbb{E}[v_{\max}]$, where $v_{\max}= \max \{v_1,\ldots,v_n\}$. However, it is not a priori clear if one can hope to come close to obtaining $\mathbb{E}[v_{\max}]$ revenue in expectation. This depends on the sharpness of the tail of the distribution of $v_{\max}$. But this may be hard to pin down, at least algorithmically, as it is the extreme value of a set of random variables. At the same time, the Statistics community has studied extreme value distributions extensively. At least for the i.i.d. case, the Fisher-Tippet-Gnedenko theorem  provides quite general conditions under which the maximum of i.i.d. random variables converges to a distribution that belongs to either the Gumbel, or the Fr\'echet, or the Weibull family of distributions. The PI and student Yang Cai~\cite{CD:multi}, exploited this theorem to pin down cases where a single price suffices for a $(1+\epsilon)$-approximation to the optimal revenue, as long as the number of items $n>g(1/\epsilon)$ for some function $g(\cdot)$. We would like to extend this result to the non-i.i.d. setting, and believe that we would have to employ interesting generalizations of the FTG theorem to do so.
\begin{theorem}[{\bf Structural 4 (i.i.d. MHR):} A Single Price Suffices for Near-Optimal Revenue] \label{thm:structural theorem 3}There is a function $g(\cdot)$ such that, for all $\epsilon>0$, if the number of items is larger than $g(1/\epsilon)$ then pricing all the items at the same price obtains a $(1-\epsilon)$-fraction of the optimal revenue, if the buyer's values are i.i.d. according to a MHR distribution.
\end{theorem} 

 \paragraph{Extreme Value Theorems.} Establishing the above structural properties relies on understanding the tails of MHR and regular distributions. For this purpose, we develop {\em extreme value theorems} for these classes of distributions. {We state our extreme value theorems informally below, referring the reader to Theorems~\ref{thm:extreme MHR} and~\ref{thm:regextremevalue} (in Sections~\ref{sec:truncate} and~\ref{sec:regular} respectively) for formal statements.}
{ 
 \begin{inftheorem}[Extreme Values of MHR Distributions]
Let $X_1,\ldots,X_n$ be a collection of independent random variables whose distributions are MHR, and let $Z=\max_i X_i$. Then, for all $\epsilon$ sufficiently small, at least a $(1-\epsilon)$-fraction of $\mathbb{E}[Z]$ is contributed to by the event $Z \le O(\log_2{1 \over \epsilon}) \cdot \mathbb{E}[Z].$
\end{inftheorem}

 \begin{inftheorem}[Extreme Values of Regular Distributions]
Let $X_1,\ldots,X_n$ be a collection of independent random variables whose distributions are regular, and let $Z=\max_i X_i$. Then the tails of $Z$ are eventually not fatter than the tails of the equal revenue distribution.\footnote{The {\em equal revenue distribution} is supported on $[1,+\infty]$ and has cumulative density function $F(x)=1-{1 \over x}$. Notice that, if a buyer's value for a single item is distributed according to this distribution, the buyer's expected value for the item is $+\infty$. However, if the item is priced at any price $x$, the expected revenue is $1$, hence the name ``equal revenue.'' {The equal revenue distribution is itself a regular distribution. So our theorem says that the tail of the maximum of $n$ regular distributions eventually behaves like the tail of a regular distribution.}}
\end{inftheorem}}
 
{Bounding the size of the tail of the {\em maximum} of $n$ independent random variables, which are MHR or regular respectively, is instrumental} in establishing the following truncation property: {restricting all the item prices into an interval of the form $[\alpha, {\rm poly}(1/\epsilon) \alpha]$ in the MHR case, and $[\alpha, {\rm poly}(n,1/\epsilon)\alpha]$ in the regular case, for some $\alpha$ that depends on the value distributions, only loses a fraction of $\epsilon$ of the optimal revenue.}~\notshow{\footnote{\yangnote{Notice that a straightforward concentration bound will only show the probability for the maximum lying outside the interval is small. However, that is not sufficient to show the contribution to the revenue from these cases is small.}}} This is quite remarkable, especially when the value distributions are non-identical or have large tails. Why can we restrict the prices into a bounded interval as above, when each of the underlying value distributions concentrates on different supports, or {even worse when they do not exhibit good concentration at all as in a power law distribution?} 

{Besides enabling the aforementioned structural results for our problem, we expect that our extreme value theorems will find applications in future work, and indeed they have already been used in followup research. In~\cite{DaskalakisW12,CaiDW12}, our theorem is used to convert nearly-optimal multi-item multi-bidder mechanisms for distributions with bounded support to nearly-optimal mechanisms for MHR distributions. For the same setting, \cite{CaiH13} use our theorem to show that relatively simple auctions can extract near-optimal revenue when the bidders are identical, by showing that the welfare is highly-concentrated.} We also note that extreme value theorems {have} been obtained in Statistics for large classes of distributions~\cite{HaanF06}, and indeed such theorems have been applied to optimal mechanism design prior to our work~\cite{BlumrosenH08}. Nevertheless, the known extreme value theorems are typically asymptotic, only hold for maxima of i.i.d. random variables, and are not known to hold for all MHR or regular distributions. We can instead handle the non-i.i.d. case, maxima of a finite number of random variables, and the full spectrum of MHR and regular distributions.


%We describe a recursive algorithm that sets up a tournament among the tails of the input distributions, and comes up with a threshold $\beta=\beta\left( \{F_i\}_i\right)$ that is within a constant factor of the optimal revenue. We then argue that a balanced interval around $\beta$ whose balance $c$ {\em only depends on $\epsilon$} contains a $(1+\epsilon)$ fraction of the revenue. The algorithm is described in Section~\ref{sec:beta} and the relation of $\beta$ to $OPT$ culminates in Theorem~\ref{lem:reduction}. The high level description of our approach is outlined in Section~\ref{sec:truncate}.

%\paragraph{Further Results.} 

\subsection{Algorithmic Ideas: Covers of Revenue Distributions} \label{sec:techniques}

We overview our approach for Theorem~\ref{thm:additive ptas}. A natural strategy for reducing the search space for an approximately optimal price vector is to discretize the set of possible prices into a finite set, whose size scales mildly with the number of items, $n$, and the approximation accuracy,~$1/\epsilon$. Of course, even with discretization the number of possible price vectors is  exponential in the number of items, and it is not clear how to search this set efficiently. A natural idea to shortcut the search further is to cluster the value distributions into a small number of buckets, containing distributions with similar statistical properties, and proceed to treat all items in a bucket as essentially identical. However, the expected revenue is not sufficiently smooth for us to perform such bucketing. We do obtain a delicate discretization of the supports of the value distributions (Corollary~\ref{cor:additive to discrete}), but cannot discretize the probabilities used by these distributions into a coarse-enough accuracy to allow for polynomial-time solvability of the problem.

Our main algorithmic idea is to shift the focus of attention from the space of {\em value distributions}, which is inherently exponential in the number of items, to the space of all possible {\em revenue distributions}, which are {\em single-dimensional} distributions. The revenue from a given price vector can be viewed as a random variable that depends on the (random) values of the items. So, there is still an exponential number of possible revenue distributions, corresponding to all possible price vectors. Nevertheless, we can exploit the single-dimensional nature of these distributions to construct a polynomial-size $\delta$-cover of the set of all possible revenue distributions under the total variation distance between distributions. That is, for every possible revenue distribution, there exists a distribution in our cover that is within $\delta$ in total variation distance from it.

Our cover is implicit, i.e. we do not provide a closed-form description for it. We show instead that it can be constructed efficiently using dynamic programming. Our algorithm iteratively considers prefixes of the items and, for each prefix $1\ldots i$, constructs a cover of all possible revenue distributions from only pricing items $1, \ldots, i$. For the next iteration, we show that the cover for items $1,\ldots,i+1$ can be easily computed from the cover for items $1,\ldots,i$ and the distribution of~$v_{i+1}$. In the end of our iterations we obtain a polynomial-size $\delta$-cover of all possible revenue distributions, and we argue that only a $\delta$-fraction of revenue is lost if we replace the optimal revenue distribution with its closest one in our cover. And, because the cover has polynomial size, we can exhaustively try every distribution in the cover and its associated price vector to pick the one with the highest expected revenue. A more detailed description of our algorithm is given in Section~\ref{sec: cover view of the problem}, and complete details are provided in Section~\ref{sec:ptas for discretized problem}. Theorem~\ref{thm:additive ptas} follows then easily in Section~\ref{sec:additive}.

Theorem~\ref{thm:general algorithm} follows similarly, except we employ a stronger discretization (Theorem~\ref{thm:discretization}) before using dynamic programming to obtain a cover of all possible revenue distributions. Finally, our algorithms for MHR and regular distributions (Theorems~\ref{thm:ptas mhr} and \ref{thm:quasi ptas regular} respectively) are corollaries of Theorem~\ref{thm:general algorithm}, except they require some extra work for restricting the value distributions into a bounded range. This is achieved in Sections~\ref{sec:truncate} (for MHR distributions) and~\ref{sec:regular} (for regular distributions) using our extreme value theorems (Theorems~\ref{thm:extreme MHR} and~\ref{thm:regextremevalue}). The detailed proofs of Theorems~\ref{thm:ptas mhr} and \ref{thm:quasi ptas regular} are provided in Appendix~\ref{sec:overall ptas}.




% There is so much that one can get from discretizations anyways$\ldots$






\notshow{\yangnote{Yang: Remove this theorem?

An interesting byproduct of our  techniques is that any constant-factor approximation to the optimal revenue can be bootstrapped to achieve an arbitrarily close approximation to it in the case of MHR and regular value distributions. This result (whose proof is given in Section~\ref{sec:overall ptas}) follows from the structure of the proof of our extreme value theorems, which can be initialized with any constant factor approximation to the optimal revenue. 
%In particular, having such approximation obviates the need to use our generic algorithm to pin down an approximation to the optimal revenue, outlined in the proofs of Theorems~\ref{thm:constant prices suffice} and~\ref{thm:logn prices suffice}.

\yangnote{Yang: Remove this theorem?}
\begin{theorem}[Constant Factor to Near-Optimal Transformation] \label{thm:constant factor to PTAS}
Given a constant-factor approximation to the optimal revenue of an instance of the pricing problem where the values are either MHR or regular, the algorithms of Theorems~\ref{thm:ptas mhr} and~\ref{thm:quasi ptas regular} can be sped up.
\end{theorem}}}

\subsection{Related and Future Work} \label{sec:related} 

%Previous work on the item pricing problem by Chawla et al.~\cite{ChawlaHK07,ChawlaHMS10} guarantees half of the optimal revenue, as long as the item values are independent. The observation enabling this result comes from an interesting comparison: Suppose that the unit-demand buyer is split into $n$ ``copies,'' $1,\ldots,n$, where copy $i$ is only interested in item $i$ and her value for that item is drawn from ${\cal F}_i$, the same distribution from which the value of the original buyer for item $i$ is drawn. The seller maintains the same feasibility constraints as before; in particular, only one item can be sold in this auction. It is intuitively obvious and can be  formally proved that the seller in the latter scenario is {better off}: there is more competition in the market, which can be exploited to extract more revenue. So the revenue of the seller in the original scenario, which we are interested in, can be upper bounded by the seller's revenue in the hypothetical scenario. In addition, the hypothetical scenario is a single-dimensional one, so we understand very well how its optimal revenue behaves by Myerson's result. With this observation in place, we can now go back to our original setting and try to come up with a price vector $P$ so that ${\cal R}_P$ approximates Myerson's revenue in the hypothetical setting, and  is hence at least as good of an approximation to the optimal revenue in the original setting. That is, we can use Myerson's revenue in the hypothetical setting as a proxy benchmark of the optimal revenue in the original setting, and our motivation for doing this is that the optimal revenue in the original (multi-dimensional) setting has no known closed-form description, while the optimal revenue in the hypothetical (single-dimensional) setting does. 
%
%Using this approach, Chawla et al.~\cite{ChawlaHMS10} specify a price vector achieving at least half of Myerson's revenue in the hypothetical scenario, and as a consequence  the revenue of the optimal price vector. Nevertheless, there is an inherent loss in their technique, as the revenue achieved by the sought-after price vector is eventually compared to a benchmark revenue that is not the optimal achievable revenue in the real setting, but the optimal revenue in the hypothetical setting, which may already be a constant factor away. So their proof technique is inherently limited to constant factor approximations due to the lack of a more accurate revenue benchmark. \yangnote{Yang: An example?}


The focus of this paper is the multidimensional item pricing problem for a unit-demand buyer whose values for the items are independent. This problem is related to the celebrated multidimensional mechanism design problem, but it is restricted in two ways. First, there is a single bidder who is unit-demand. Second, we are interested in coming close to the revenue of the optimal {\em deterministic}---i.e. item pricing---mechanism and not the optimal unrestricted  mechanism, which may also price lotteries over items. While it is unclear whether the restriction to deterministic mechanisms should make the problem easier or harder computationally, the restriction to a single unit-demand bidder should make the problem easier compared to having many bidders with arbitrary valuations.

Despite the apparent simplicity of the item pricing problem,  (near-)optimal polynomial-time algorithms for it were not known prior to our work. Chawla et al.~\cite{ChawlaHK07} provide a  $3$-approximation algorithm, computing a price vector whose revenue is at least a third of the optimal revenue. Their technique is quite elegant, connecting the item pricing problem to a related, single-dimensional mechanism design problem, which can be analyzed using Myerson's result~\cite{Myerson81}. Using the same approach, the approximation factor is improved to $2$ in~\cite{ChawlaHMS10}, and the result is generalized to the multi-bidder setting, albeit with a worse approximation factor. Different work~\cite{BhattacharyaGGM10,Alaei11} obtains polynomial-time constant factor approximations for additive bidders, using convex programming relaxations of the problem. 

However, all these approaches are limited to constant factor approximations, as ultimately the attained revenue is compared to the optimal revenue in a related single-dimensional setting~\cite{ChawlaHK07,ChawlaHMS10}, or a convex programming relaxation of the problem~\cite{BhattacharyaGGM10,Alaei11}. In particular, the limitation of these approaches comes from avoiding a direct comparison of the attained revenue to the optimal revenue in the actual problem, comparing it instead to the optimal revenue in a related problem. Our work provides instead near-optimal algorithms, using a direct comparison to the real optimum via covers of revenue distributions. 

Our work leaves several directions open for exploration and some have already been studied following the announcement of our results~\cite{CaiD11}. We classify them into three categories discussed below.
\begin{itemize}
\item {\em Unit-demand Bidders:} Can our near-optimal algorithms be improved to be exactly optimal? Recent work has shown that the answer is no, namely that there are no exactly optimal polynomial-time  algorithms for product value distributions, unless ${\tt P} = {\tt NP}$~\cite{ChenDPSM14}. Still there is room for improving the dependence of our running times on the approximation parameter $\epsilon$. E.g., is there an algorithm that runs in time polynomial in $n$ and $1/\epsilon$ when the item values are bounded in~$[0,1]$?

And how about correlated distributions over item values? Here, it had already been known that computing an optimal price vector is highly inapproximable in polynomial-time~\cite{BriestK07}. So there cannot even be a polynomial-time constant factor approximation in this case.

Beyond item pricing, it is important to understand the complexity of optimal randomized mechanisms, which may increase revenue by also pricing lotteries over items~\cite{Thanassoulis04,BriestCKW10}. For product distributions, Chawla et al.~\cite{ChawlaMS10} {show that randomization does not increase revenue by more than a factor of 4, thus extending} the constant-factor approximation algorithms of~\cite{ChawlaHK07,ChawlaHMS10} to the randomized multi-bidder setting, except with worse approximation guarantees. Is there a polynomial-time optimal mechanism for this setting? No computational lower bound is known at the time of writing of this paper. 

For correlated distributions over item values, Cai et al.~\cite{CaiDW12b} obtain near-optimal, randomized mechanisms for multi-bidder multi-item settings with unit-demand bidders. For any desired accuracy $\epsilon>0$, they compute a mechanism whose revenue is within an additive error of $\epsilon$ from optimal in time polynomial in $1/\epsilon$ and the size of the support of each bidder's distribution over valuations, {when these distributions are discrete. (When they are continuous, they are handled via fine enough discretization.)} This algorithm is clearly also applicable  when every bidder's values for the items are independent (i.e. the setting discussed in the previous paragraph). However, the dependence of the running time on the support of the product distribution may be unreasonable computationally. Indeed, a {discrete} product distribution can be described by specifying all of its marginals, with description complexity logarithmic in the size of its support. 
%
%While this is the best possible when the item-values are correlated, it may be suboptimal when (as in our case) the values  are independent, as the distribution may then have support of size exponential in its description complexity. For example, if a bidder's values for the items are independent and supported on a set of cardinality $2$, then the bidder's value distribution will have support of size exponential in the number of items, and the number of bits required to describe the distribution. So the mechanism of Cai et al.~\cite{CaiDW12,CaiDW12b} will run in time exponential in the number of items, not achieving the polynomial dependence of the running time in the number of items achieved by our results.


\item {\em Additive Bidders:} Can our algorithms be extended to additive bidders? Here, an optimal mechanism may increase revenue by pricing bundles of items~\cite{ManelliV06}, or (if randomization is allowed) lotteries over bundles of items. Exploiting our extreme value theorems for MHR distributions, Cai and Huang~\cite{CaiH13} provide near-optimal polynomial-time mechanisms for multiple i.i.d. bidders, whose values for the items are independently distributed according to MHR distributions. Moreover, Daskalakis et al.~\cite{DaskalakisDT14} show that this result cannot be made exact for general product distributions. They show that, subject to widely held complexity theoretic beliefs---in particular that ${\tt ZPP} \not\supseteq {\tt P}^{\#{\tt P}}$,\footnote{${\tt ZPP} \supseteq {\tt P}^{\#{\tt P}}$ would imply that there are randomized polynomial-time algorithms for ${\tt NP}$-complete problems, which is widely believed to be unlikely.} computing and implementing an exactly optimal mechanism cannot be done computationally efficiently. Indeed, this is true even in the ostensibly simple setting where there is a single additive bidder whose values for the items are independently distributed on two rational numbers with rational probabilities. 

For correlated distributions, Cai et al.~\cite{CaiDW12} obtain (exactly) optimal mechanisms for multi-bidder multi-item settings with additive bidders, in time polynomial in the size of the support of each bidder's distribution over valuations.

On a different vein, Daskalakis et al.~\cite{DaskalakisDT13} study the structure (rather than the computational complexity) of optimal mechanisms, following earlier work on the topic by Economists, e.g.~\cite{Rochet85,Armstrong00,ManelliV06,ManelliV07,Pavlov11}. They provide a duality framework  based on Monge-Kantorovich duality for characterizing the structure of the optimal mechanism of selling multiple items to a single additive bidder.

%Armstrong96,Mcafee88,


\item {\em General Settings:}\notshow{\yangnote{\footnote{\yangnote{Yang says: I think going directly to general objective might be too big a jump for the readers. Can we talk about revenue with general valuations first, then go to general objectives? Also, I think we should specifically point out that for revenue the algorithmic problem is only maximizing welfare. I am worried that the readers will think revenue plus welfare is not a well defined objective (e.g. under what constraints?)...}}}} It is important to understand the computational complexity of mechanism design in general settings: multiple bidders, general valuations {(beyond unit-demand and additive), general constraints on what allocations of items to bidders are feasible,} and general objectives, potentially going beyond the familiar objectives of revenue and welfare.\footnote{{A general objective $O$ takes as input the valuations of the bidders $\vec{t}$ and a randomized allocation and price vector $(A,p)$ and outputs a real number $O(\vec{t},(A,p))$.}} In recent work, Cai et al.~\cite{CaiDW13b} provide a {computational black-box reduction from {\em mechanism design} for maximizing an arbitrary concave objective $O$\footnote{{An objective function $O(\vec{t},(A,p))$ is called {\em concave} iff, for all bidder valuations $\vec{t}$, and all $(A_1,p_1)$ and $(A_2,p_2)$, it holds that $O(\vec{t}, {1 \over 2} (A_1,p_1) + {1 \over 2}  (A_2, p_2)) \ge {1 \over 2}  O(\vec{t}, (A_1, P_1)) + {1 \over 2}  O(\vec{t}, (A_2, P_2))$, where ${1 \over 2}  (A_1,p_1) + {1 \over 2}  (A_2, p_2)$ denotes uniformly randomizing between $(A_1,p_1)$ and $(A_2,p_2)$. Clearly, revenue and welfare satisfy this condition with equality, but several other objectives are concave, such as the max-min fairness objective considered in~\cite{CaiDW13b}.}} under arbitrary allocation constraints and an arbitrary family of bidder valuations (e.g. submodular, supermodular, etc.) to {\em algorithm design} for that same objective $O$, modified by an additive virtual welfare term, and under the same allocation constraints and family of allowed valuations.} Roughly speaking, they show that, whenever the algorithmic problem is polynomial-time solvable (exactly or approximately), the mechanism design problem also becomes solvable (exactly or approximately) in time polynomial in the size of the support of each bidder's distribution over valuations. It is important to find applications of this reduction to settings of interest beyond optimizing fractional max-min fairness for additive bidders, which was done in~\cite{CaiDW13b}.

%It is also important to extend our results to the multi-bidder problem, extending Myerson's  auction to the multidimensional setting, and the results of~\cite{BhattacharyaGGM10,ChawlaHMS10,Alaei11} to beyond constant factor approximations. In recent work, Daskalakis and Weinberg~\cite{DaskalakisW11} have made progress on this front obtaining near-optimal, computationally efficient, randomized mechanisms for multi-bidder multi-item auctions, when either the number of bidders is an absolute constant and the value distribution is item-symmetric, or the number of items is an absolute constant and the value distribution is bidder-symmetric. Hence, these results do not imply ours, as we are not making any item-symmetry assumption. Even more recently, Cai et al.~\cite{CaiDW12,CaiDW12b}  
\end{itemize}


 

%We also leave the complexity of the exact problem as an open question, and conjecture that it is $NP$-hard, referring the reader to~\cite{BK} for hardness results in the case of correlated distributions. 



%It remains open whether near-optimal randomized mechanisms for the multi-item multi-bidder problem exist, which run in time polynomial in both the number of items and the number of bidders.

%. These results are neither subsumed, nor subsume the results in the present paper. Indeed, we are more general here in that we allow the buyer to have values for the items that are not necessarily i.i.d., an assumption needed in~\cite{DW} if the number of items is large. On the other hand, we are less general in that (a) we solve the single-bidder problem and (b) are near-optimal with respect to all deterministic (i.e. item pricing), but not necessarily randomized (lottery-pricing) mechanisms. Strikingly, the techniques of the present paper are essentially orthogonal to those of~\cite{DW}. The approach of~\cite{DW} uses randomness to symmetrize the solution space, coupling this symmetrization with Linear Programming formulations of the problem. Our paper takes instead a probabilistic approach, developing extreme value theorems to characterize the optimal solution, and designing covers of revenue distributions to obtain \yangnote{computationally} efficient algorithmic solutions. It is tempting to conjecture that our approach here, combined with that of~\cite{DW} would lead to more general results. Indeed, our extreme value theorems found use in~\cite{DW}, but we expect that significant technical work is required to go forward.
%
% 
%
%It would be cool to extend to many bidders. Daskalakis + Weinberg for symmetric. Then Cai+Daskalakis+Weinberg for general but running time exponential in the number of items (polynomial in the number of bidders)


%We believe that our extreme value theorems, and our probabilistic view of the problem in terms of revenue distributions will be helpful in obtaining more general results. 




%In conclusion, this paper provides the first near-optimal \yangnote{computationally}  efficient algorithms for interesting instances of the multidimensional mechanism design problem, for a unit-demand bidder whose values are independent (but not necessarily identically distributed.) Our results provide algorithmic, structural and probabilistic insights into the properties of the optimal deterministic mechanism for the case of MHR, regular, and more general distributions. 

%
%Of course, it would be important to obtain black-box type results for the pricing/optimal mechanism design problem, such as those that have been developed for optimizing the social welfare~\cite{HL,HKM,BH,DR}.


==> non-iid_OLD.tex <==




\section{Probabilistic Covers of Revenue Distributions} \label{sec: cover view of the problem}


%It follows from Lemma~\ref{lem:horizontal-discretization} that, given any collection of mutually independent random variables $\{v_i\}_{i \in [n]}$ representing the buyer's values for the items (where these random variables may be supported on a continuum of points), we can efficiently construct\footnote{We postpone issues of numerical accuracy to the next section.} a collection of mutually independent random variables $\{\hat{v}_i\}_{i \in [n]}$ of finite support and reduce the search for an optimal price vector under buyer values $\{v_i\}_{i \in [n]}$ to the search of an optimal price vector under buyer values $\{\hat{v}_i\}_{i \in [n]}$. For some {\color{red}$\delta \in (0,\frac{1}{(4 \lceil \log r\rceil) ^{4/3}})$}, let us denote by $\{\hat{F}_i\}_{i\in[n]}$ the set of distributions obtained from $\{{F}_i\}_{i\in[n]}$ via an application of Lemma~\ref{lem:horizontal-discretization}. Replacing $\{{F}_i\}_{i\in[n]}$ by $\{\hat{F}_i\}_{i\in[n]}$ only loses a $\delta$ fraction of the revenue. For convenience, we denote by $\{v^{(1)},v^{(2)},\ldots,v^{(k_1)}\}$ the support of the distributions $\{\hat{F}_i\}_{i\in[n]}$ given by Lemma~\ref{lem:horizontal-discretization}, and we note that {\color{red} $k_1 = O(\frac{\log r}{\delta^2})$}. 
%
%Moreover, Lemma~\ref{lem:betweenminmax} and Proposition~\ref{cor:discreteprice} imply that we only lose an $\epsilon$ fraction of the optimal revenue if we restrict our attention to a finite set of prices $\{p^{(1)}, p^{(2)},\ldots, p^{(k_2)}\}$, of cardinality {\color{red} $k_2=O({\log r \over \epsilon^2})$}. It is worth noting that this set of prices satisfies $\min\{p^{(i)}\} \ge u_{min}/(1+\epsilon)$ and $\max\{p^{(i)}\} \le u_{max}$, and the prices in the set are points of a geometric sequence of ratio $1/(1-\epsilon^2)$.
%
%Let us denote by $\hat{\cal R}_{OPT}$ the optimal revenue achieved when the buyer's values  are distributed as $\{\hat{v}_i\}_{i\in[n]}$ and we are only allowed to use prices from the set $\{p^{(1)}, p^{(2)},\ldots, p^{(k_2)}\}$.  The above discussion argues that {\color{red}$\hat{\cal R}_{OPT} \ge \big{(}1-O(\epsilon+\delta^{1/8})\big{)} {\cal R}_{OPT}$}, where ${\cal R}_{OPT}$ is the optimal revenue for the original value distributions and without restrictions on the set of prices.

\notshow{\yangnote{Let ${\cal V}:=\{v_i\}_{i}$ be an instance of {\sc AdditivePrice}, where the $v_i$'s are mutually independent random variables distributed  on $[0,1]$ according to the distributions $\{{F}_i\}_{i}$, and let ${\cal R}_{OPT}$ be the expected revenue from the optimal price vector for $\cal V$. Our goal in this section is to compute a price vector with expected revenue at least ${\cal R}_{OPT}-\epsilon$. 

Section~\ref{sec:additive} provides a {computationally} efficient reduction of this problem to the problem of approximating within additive $O(\epsilon)$ of the optimal revenue of a discretized problem, where both the values and the prices come from discrete sets whose cardinality is $O({{\log 1/\epsilon}\over{\epsilon^2}})$. 

To accommodate scenarios that will be considered in future sections, we provide a more general algorithm. We assume the values lie in an interval $[u_{min},u_{max}]$ where $r = {u_{max} \over u_{min}}$. For convenience, we denote by $\{\hat{F}_i\}_i$ the discretized distributions resulting from the reduction, by $\{\hat{v}_i\}_{i}$ a collection of mutually independent random variables distributed according to the $\hat{F}_i$'s, by $\{v^{(1)},v^{(2)},\ldots,v^{(k_1)}\}$ the (common) support of all the $\hat{F}_i$'s, and by $\{p^{(1)}, p^{(2)},\ldots, p^{(k_2)}\}$ the set of available price levels, where for {\sc RestrictedPrice}$(\mathcal{\hat{V}},\mathcal{P},O(\epsilon))$ in Corollary~\ref{cor:additive to discrete} both $k_1$ and $k_2$ are $O({{\log 1/\epsilon}\over{\epsilon^2}})$. %It is worth pointing out that the reduction of Theorem~\ref{thm:discretization} satisfies the following property: the set of prices satisfies $\min\{p^{(i)}\} \ge u_{min}/(1+\delta)$ and $\max\{p^{(i)}\} \le u_{max}$, and these prices are points of a geometric progression of ratio $1/(1-\delta^2)$. (See Lemmas~\ref{lem:betweenminmax} and~\ref{cor:discreteprice} in Section~\ref{sec:discretizing prices}.)
}}

In this section, we discuss our algorithmic approach to {\scshape RestrictedPrice}, postponing the description of our algorithm for it to Section~\ref{sec:ptas for discretized problem}. As we have already discussed in Section~\ref{sec:proof outline}, although seemingly restricted this problem captures the main algorithmic challenges underlying  problems {\scshape Price} and {\scshape AdditivePrice}. In particular, our algorithm for {\scshape RestrictedPrice} will become a central building block in all our algorithmic results (Theorems~\ref{thm:additive ptas} through~\ref{thm:quasi ptas regular}). 

For convenience, throughout this section we will take ${F}_1,\ldots,{F}_n$ to be a collection of distributions supported on a discrete set ${\cal S}=\left\{v^{(1)},v^{(2)},\ldots,v^{(k_1)}\right\}$, and ${v}_1,\ldots,{v}_n$ to be a collection of mutually independent random variables distributed according to the ${F}_i$'s. We will then assume that the  input to {\scshape RestrictedPrice} comprises the ${v}_i$'s and a finite set of prices ${\cal P}=\{p^{(1)}, p^{(2)},\ldots, p^{(k_2)}\}$.

\smallskip The obvious algorithmic challenge in {\sc RestrictedPrice} is that, even though the set of possible prices is finite, there are still exponentially many (namely $k_2^n$) possible price vectors that we need to choose from for an optimal one. If $k_2$ were a constant and the items were i.i.d., then we could decrease the possible vectors to a polynomial number by exploiting the symmetry of the items.\footnote{A broader exposition of the role of symmetries in mechanism design can be found in~\cite{DaskalakisW12}.} Similarly, we can obtain polynomial-time algorithms for the case where there is only a constant number of possible value distributions and a constant number of possible prices. However, when all the $F_i$'s may be different, the problem looks inherently exponential, even if both $k_1$ and $k_2$ are absolute constants, e.g., even when the value distributions are supported on $2$ possible values and there are $2$ possible prices available.

%
% natural algorithmic approach is to try to decrease the set of possible inputs to {\sc R}
%
%
%Even though the distributions input to our problems have 
%
%
%Facing distributions with discrete supports and a discrete set of possible prices, a natural approach is to try to decrease the set of possible inputs to the problem. In particular, it is natural to try and further discretize the distributions $\hat{F}_1,\ldots,\hat{F}_n$ by rounding the probabilities they assign to every point in their support to integer multiples of some fraction $\sigma >0$. If both $\sigma$ and $k_1$ depended only mildly on the parameters of the problem, then the number of possible distributions would only be a function of $\epsilon$
%one would hope that the number of possible value distributions would only be a function of
%
%
%$=\sigma(\epsilon)>0$, i.e. a fraction that does not depend on $n$ but potentially depends on $\epsilon$. If such discretization were feasible, the number of possible distributions would only be a function of $\epsilon$. In such a case, we could try to develop an algorithm tailored to a small number of possible value distributions. This is still not easy to do (as even the i.i.d. case of our problem poses challenges), but is definitely  an easier computational problem. Nevertheless, the approach breaks down as preserving the revenue while doing a coarse rounding of the probabilities appears difficult, and the best discretization we can obtain is given in Lemma~\ref{lem:verticaldiscretization} of Appendix~\ref{sec:vertical discretizing values}, where the accuracy is inverse polynomial in the number of items $n$. 


%the problem would be greatly simplified. For example, if $r$ were an absolute constant or a function of $\epsilon$ only (as it happens \yangnote{for the additive approximation after applying Theorem~\ref
%{thm:additive discretization} in Section~\ref{sec:additive}} \notshow{and for MHR distributions after applying the reduction of Theorem~\ref{thm:reduction MHR to balanced}}), there would only be a constant number of possible value distributions (as both the cardinality of the support of the distributions and the number of available probability levels would be a function of $\epsilon$ only.) 

Our algorithmic approach is enabled by a shift in perspective, which may be applicable to other problems with a similar structure. To illustrate the approach, let us view our problem in the graphical representation of Figure~\ref{fig:d1}. $C$ is a function that takes as input a price vector $P=(p_1,\ldots,p_n)$ and outputs the distribution ${F}_{{ R}_P}$ of the revenue of the seller under this price vector. Indeed, the revenue of the seller is a random variable ${R}_P$ that depends on the random variables $\{{v}_i\}_{i \in [n]}$. So in order to compute the distribution of the revenue, $C$ also takes as input the distributions $F_1,\ldots,F_n$. What we are aiming at maximizing is the expectation ${\cal R}_P$ of of ${R}_P$.
\begin{figure}[h!]
  \centering
  \includegraphics[height = 1.4in]{circuit.pdf}\\
   \caption{The Revenue Distribution as the output of a function. The inputs to the function are the prices and the value distributions.}\label{fig:d1}
\end{figure}
 
Given our restriction of the prices to a finite set $\{p^{(1)}, p^{(2)},\ldots, p^{(k_2)}\}$, there are $k_2^n$ possible inputs to the circuit, and at most $k_2^n$ possible revenue distributions that the circuit can produce. Our main conceptual idea is the following:\\ 

\begin{minipage}[h]{15cm}{\em Instead of searching the space of possible price vectors that can be input to $C$, we search the space of possible outputs of $C$, i.e. the space of all possible revenue distributions resulting from different price vectors, for one with maximum expectation.

\smallskip Moreover, to efficiently search the space of all possible revenue distributions, we construct an appropriately small subset of it and only search the distributions in that subset.}\end{minipage}

\bigskip \noindent The subset we construct is a probabilistic cover (under some appropriate metric) of the space of all possible revenue distributions.\footnote{A {\em $\delta$-cover} of a set of distributions ${\cal F}$ with metric $d$ is a subset ${\cal F}' \subseteq {\cal F}$ such that for all $F \in {\cal F}$ there exists some $F' \in {\cal F}'$ such that $d(F,F') \le \delta$.} The properties of our cover that are crucial for our algorithmic applications are the following: (a) the cover has cardinality \costasnote{$O(n^{{\rm poly}({1 \over \epsilon},\log r)})$, where $r=\max_{i,j}\left\{{p^{(j)} \over p^{(i)}}\right\}$}, and (b) for any possible revenue distribution that the circuit may output, there exists a revenue distribution in our cover with approximately the same expectation. 

\paragraph{Constructing the Cover.} At a high level, we construct our cover using dynamic programming, whose steps are interleaved with coupling arguments that prune the size of the DP table before proceeding to the next step. 

\smallskip Intuitively, our dynamic program sweeps the items from $1$ through $n$, maintaining a cover of the revenue distributions produced by all possible price vectors on every prefix of the items. More precisely, for each prefix $1\ldots j$ of the items, our DP table keeps track of all possible feasible collections of $k_1\times k_2$ probability values, where $\Pr_{i_1,i_2}$, $i_1 \in [k_1], i_2 \in [k_2]$, denotes the probability that the item with the largest value-minus-price gap (i.e. the item that would have been sold in a sale that only sells items $1$ through $j$) has value $v^{(i_1)}$ for the buyer and is assigned price $p^{(i_2)}$ by the seller. I.e. we store in our DP table all possible (winning-value, winning-price) distributions that can arise from a price vector on every every prefix of the items. The reasons we store these distributions are the following:
\begin{itemize}

\item First, if we have all possible (winning-value, winning-price) distributions for the full set of items, we can search for the one with the highest expected revenue. For every distribution we will also maintain in our DP table a price vector resulting in that distribution. So, once we have found the distribution with the optimal expected revenue, we will also find the price vector with that optimal revenue.

\item Second, we can construct the set of all possible (winning-value, winning-price) distributions for the full set of items, by considering one prefix at a time. In particular, suppose that we have all possible (winning-value, winning-price) distributions for the prefix of items $1\ldots j$. By combining every such distribution with all $k_2$ possible prices for item $j+1$, we can compute all possible (winning-value, winning-price) distributions for the prefix of items $1\ldots j+1$. That is, if we have these distributions for a prefix of items, we do not need any other information to extend the prefix by one item. For this scheme to work, observe that it is crucial to maintain the joint distribution of both the winning-value and the winning-price, rather than just the distribution of the winning-price.

%As we sweep through the items, we have $k_2$ possible prices we can assign to the next item. 
%
%, when our dynamic program considers assigning a particular price to the next item, then having the  (winning-value, winning-price) distribution on the prefix suffices to obtain the new (winning-value,winning-price) distribution that also includes the next item at the chosen price. 
%
%\item First, for every such distribution, we can compute the expected revenue of the seller, if the sale is restricted to that prefix of items.
%
%
%
%\item Finally, if we have all possible (winning-value, winning-price) distributions for the full set of items, we can search for the one with the highest expected revenue. Then we can follow back-pointers stored in our DP table to uncover a price vector consistent with the optimal distribution.
\end{itemize}

Clearly, the dynamic programming approach that we just outlined for computing a cover of all possible revenue distributions achieves nothing in terms of reducing the number of distributions. Indeed, there could be one (winning-value, winning-price) distribution for every price vector, so that the total number of distributions that we need to store in our DP table is exponential. To control the size of our cover from exploding, we show that we can be coarse in our bookkeeping of the (winning-value, winning-price) distributions, without sacrificing much revenue. Indeed, it is here where viewing our problem in the ``upside-down'' manner illustrated in Figure~\ref{fig:d1} (i.e. targeting a cover of the output of $C$) is important. We show that we can discretize the probabilities used by the distributions stored in the DP table into multiples of \costasnote{$1\over (nr)^{3}$} without losing much revenue. In particular, after a prefix of items is processed by the dynamic program, we show that we can discretize the probabilities in all distributions in the table before considering the next item. That the loss due to coarsening the probabilities is not significant follows from coupling arguments interleaved with the steps of the the dynamic program.


%As the dynamic program is unraveling, we show ta
%
%After every step of the dynamic programming algorithm we can discretize the probabilities used in the maintained distributions into multiples of 
%We show that we can discretize 
%
%, after each step of our dynamic programming algorithm (i.e. after a prefix is completely processed), we can discretize all probabilities used in our distributions into multiples of $1\over (nr)^{3}$ without losing much revenue, and while keeping the size of the DP table from exploding. 

\medskip In the next section we make our ideas precise, obtaining our algorithm for {\sc RestrictedPrice}.


%More precisely, for each prefix of the items, our DP table keeps track of the following information: 
%\begin{enumerate}
%
%\item all possible records of how many items in the prefix have been assigned each of the available prices $p^{(1)}, p^{(2)},\ldots, p^{(k_2)}$;
%
%\item all possible feasible collections of $k_1\times k_2$ probability values, where $\Pr_{i_1,i_2}$, $i_1 \in [k_1], i_2 \in [k_2]$, denotes the probability that the item with the largest value-minus-price gap (i.e. the item of the prefix that would have been sold in a sale that only sales the prefix of items) has value $v^{(i_1)}$ for the buyer and is assigned price $p^{(i_2)}$ by the seller.
%\end{enumerate}
%%During this procedure, we will record for each price, how many items have been assigned to this particular price. And another $k_1k_2$ probabilities. We use ${\Pr}_{i_1,i_2}$ to denote the $i_1\cdot k_1+i_2$-th probability we recorded, ${\Pr}_{i_1,i_2}$ is the probability that the item, which has the largest gap between its value and price, has value $v^{(i_1)}$ and price $p^{(i_2)}$. 
%In other words, for every prefix of items and for every possible signature of how many items of the prefix have been given each of the available $k_2$ prices, we memoize all possible (winning-value, winning-price) distributions that can arise from that prefix and that signature. There are two reasons we want to memoize these distributions:
%\begin{itemize}
%\item first, if we have these distributions, we can compute the expected revenue that the seller would obtain, if we restricted our sale to the prefix of items; 
%
%\item second, when our dynamic program considers assigning a particular price to the next item, then having the  (winning-value, winning-price) distribution on the prefix suffices to obtain the new (winning-value,winning-price) distribution that also includes the next item; i.e., if we have these distributions, we do not need to keep track of anything else in the history to keep going.
%
%\item in the end of the program, we can look at all feasible (winning-value,winning-price) distributions for the full set of items to find out which achieves the best revenue; we can then follow back-pointers to find a price vector consistent with the distribution that we selected.
%\end{itemize}
%
%\noindent All this sounds reasonable, and fun, but thus far we haven't achieved anything in terms of reducing the number of distributions $F_{\hat{{R}}_p}$ in our cover. Indeed, there could be many (winning-value,winning-price) distributions consistent with each signature, so that the total number of distributions that we have to memoize in the course of the algorithm is exponentially large. To obtain a polynomially small cover we show that we can be coarse in our bookkeeping of the (winning-value, winning-price) distributions, without sacrificing much revenue. Indeed, it is exactly here where viewing our problem in the ``upside-down'' way illustrated in Figure~\ref{fig:d1} (i.e. targeting a cover of the output of circuit $C$ rather than figuring out a sparse cover on the input) is important: we show that, as far as the expected revenue is concerned, we can discretize probabilities into multiples of $1\over (nr)^{3}$ after each round of the DP without losing much revenue and while keeping the running time of the DP from exploding. That the loss due to pruning the search space is not significant follows from a double application of the coupling lemma and the optimal coupling theorem (see, e.g.,~\cite{durrett2}), after each step of the Dynamic Program.

%It is On the other hand, while discretizing the input distributions into multiples of %$1/n^3$
%{\color{red} $1\over (nr)^{3}$} does not hurt the revenue (Lemma~\ref{lem:verticaldiscretization}), it nevertheless keeps the search space exponentially large. 
% of possible input/output distributions of the circuit exponential.

%It is not hard to see that if in every step we can record the probabilities accurately, we only need to exhaustive search for all possibilities then we can find the optimal solution. However, we can not afford to record the probabilities accurately, since this will give us exponentially many possible outcomes. So what we do is in every step, we round the probabilities into an integer multiple of $1/n^3$. We will show that by rounding the probabilities, we only lose a negligible fraction of the revenue. 

\section{The Algorithm for the Discrete Problem} \label{sec:ptas for discretized problem}
%For this balanced case of our problem,
%{\color{red} For simplicity, we let $m=nr$.}


In this section, we formalize our ideas from the previous section, describing our main algorithmic result for {\sc RestrictedPrice}. We use the same notation as in Section~\ref{sec: cover view of the problem}, namely we assume that the input distributions are supported on a common set ${\cal S}$ of cardinality $k_1$ and the prices are restricted to a set ${\cal P}$ of cardinality $k_2$. We also denote by $OPT$ the optimal expected revenue for the input value distributions when the prices are restricted to ${\cal P}$.

%We assume that the pricing problem at hand is discrete: the value distributions are supported on a discrete set ${\cal S}=\{v^{(1)},v^{(2)},\ldots,v^{(k_1)}\}$, and the sought-after price vector also lies in a discrete set $\left\{p^{(1)},\ldots,p^{(k_2)}\right\}^n$, where both $\cal S$ and ${\cal P}=\left\{p^{(1)},\ldots,p^{(k_2)}\right\}$ are given explicitly  as part of the input, while our access to the value distributions may still be either explicit or via an oracle. We denote by ${OPT}$ the optimal expected revenue for this problem, when the prices are restricted to set  $\cal P$. %It is $OPT$ that are looking to approximate.

%, where both $k_1$ and $k_2$ are $O(\log r/\delta^2)$, $\delta=O(\epsilon^8)$ and the discrete sets where the values and the prices lie are explicitly given as part of the input. This discrete problem is the problem we are looking to solve; 
\paragraph{The Algorithm.} As a first step we discretize the probabilities used by the input distributions. We prove a discretization lemma that provides a polynomial-time reduction from our problem into a new one, where additionally the probabilities that the value distributions assign to each point in ${\cal S}$  are integer multiples of $1/m^3$, where $m:=\lceil \frac{nrk_{1}k_{2}}{\epsilon}\rceil$ and $r=\max_{i,j}\left\{{p^{(j)} \over p^{(i)}}\right\}$; see Lemma~\ref{lem:verticaldiscretization} in Appendix~\ref{sec:vertical discretizing values}. We show that the loss in revenue resulting from our reduction is at most an additive {$\frac{4k_1nr}{m^3} \min_i\{p^{(i)}\}$}. Moreover, the construction of Lemma~\ref{lem:verticaldiscretization} is explicit, so from now on we can assume that we know the value distributions explicitly. Let us denote by $\{\hat{F}_i\}_i$ the discretized distributions. 


%on the value distributions $\{{F}_i\}_{i}$, modifying them into new value distributions $\{{F}_i\}_{i}$ so that each point in their support receives probability that is an integer multiple of $1/(rn)^3$, where $r=\max\left\{{p^{(j)} \over p^{(i)}}\right\}$. 
%In this section, we formalize our ideas from the previous section, providing our main algorithmic result. We assume that our original pricing problem {\sc OptPrice}$({\cal V},\epsilon)$ has been reduced to the $(1-\delta)$ approximation of a discrete problem, whose value distributions $\{\hat{F}_i\}_i$ are supported on a discrete set $\{v^{(1)},v^{(2)},\ldots,v^{(k_1)}\}$ and the sought after price vector also lies in a discrete set $\left\{p^{(1)},\ldots,p^{(k_2)}\right\}^n$, where both $k_1$ and $k_2$ are $O(\log r/\delta^2)$, $\delta=O(\epsilon^8)$ and the discrete sets where the values and the prices lie are explicitly given as part of the input. This discrete problem is the problem we are looking to solve; we denote its optimal expected revenue by $\widehat{OPT}$. 
%
%Before proceeding, we invoke Lemma~\ref{lem:verticaldiscretization} on the distributions $\{ \hat{F}_i\}_{i}$, modifying them so that each point in their support receives probability that is an integer multiple of $1/(rn)^3$. Lemma~\ref{lem:verticaldiscretization} guarantees that the loss in revenue from this modification is at most an additive $\frac{4k_1}{rn^2} \min\{p^{(i)}\}$. Moreover, the construction of Lemma~\ref{lem:verticaldiscretization} is explicit, so from now on we can assume that we know the distributions $\{ \hat{F}_i\}_i$ explicitly. Moreover, we set $m:=r n$ throughout this section for notational convenience.

The second phase of our algorithm is the Dynamic Program outlined in Section~\ref{sec: cover view of the problem}. We provide some further details on this next. Our program computes a Boolean function $g(i,{\widehat{\Pr}})$, whose arguments lie in the following range:  $i\in[n]$ and ${\widehat{\Pr}}=(\widehat{\Pr}_{1,1},\widehat{\Pr}_{1,2},\ldots,\widehat{\Pr}_{k_1,k_2})$, where each $\widehat{\Pr}_{i_1,i_2} \in [0,1]$ is an integer multiple of {$1\over m^3$}. The function $g$ is stored in a table that has one cell for every setting of $i$ and ${\widehat{\Pr}}$, and the cell contains a $0$ or a $1$ depending on the value of $g$ at the corresponding input. In the terminology of the previous section, argument $i$ indexes the last item in a prefix of items and ${\widehat{\Pr}}$ defines a (winning-value, winning-price) distribution whose probabilities are integer multiples of ${1 \over m^3}$. If ${\widehat{\Pr}}$ can arise from some pricing of the items $1 \ldots i$ (up to discretization of probabilities into multiples of ${1 \over m^3}$), we intend to store $g(i,{\widehat{\Pr}})=1$; otherwise we store $g(i,{\widehat{\Pr}})=0$.

For coherence, we give next a high-level description of the dynamic program, postponing its details to Section~\ref{sec:DP step}. The table is filled in a bottom-up fashion from $i=1$ through $n$. At the end of the $i$-th iteration, we have computed all feasible ``discretized'' (winning-value,winning-price) distributions for the prefix of items $1\ldots i$, where ``discretized'' means that all probabilities have been rounded into multiples of $1/m^3$. For the next iteration, we try all possible prices $p^{(j)}$ for item $i+1$ and compute how each of the feasible discretized (winning-value,winning-price) distributions for the prefix $1\ldots i$ evolves into a discretized distribution for the prefix $1\ldots i+1$, setting the corresponding cell of layer $g(i+1,\cdot)$ of the DP table to $1$. Notice, in particular, that {\em we lose accuracy in every step of the Dynamic Program}, as each step involves computing how a discretized distribution for items $1\ldots i$ evolves into a distribution for items $1\ldots i+1$ and then rounding the latter back into multiples of $1/m^3$. We show in the analysis of our algorithm that the error accumulating from these roundings can be controlled via coupling arguments.

After computing the truth-table of function $g$, we look at all cells such that $g(n,\widehat{\Pr})=1$ and evaluate the expected revenue resulting from the distribution $\widehat{\Pr}$, i.e.
$${\cal R}_{\widehat{\Pr}} = \sum_{i_1\in[k_1],i_2\in[k_2]} p^{(i_2)}\cdot \widehat{\Pr}_{i_1,i_2} \cdot \ind_{v^{(i_1)}\geq p^{(i_2)}}.$$
Having located the cell whose ${\cal R}_{\widehat{\Pr}}$ is the largest, we follow back-pointers to obtain a price-vector consistent with $\widehat{\Pr}$. At some steps of the back-tracing, there may be multiple choices; we pick an arbitrary one to proceed.



%Of course, since our accuracy in the DP table is not infinite,  before turning bits to $1$ we {\em round the distributions in some canonical way so that all probabilities are integer multiples of $1/m^3$.} We also use back pointers to remember what cell of layer $g(i,\cdot)$ and what price $p^{(j)}$ for item $i+1$ brought us here. However,    since our accuracy in the DP table is finite,
%Note that we are throwing away information by only remembering

%Intuitively, we want $g(i,C_1,C_2,\ldots,C_{k_2},\widehat{\Pr}_{1,1},\widehat{\Pr}_{1,2},\ldots,\widehat{\Pr}_{k_1,k_2})$ equals $1$ if and only if there is a partial price vector $(p_1,p_2,\ldots,p_i)$ for the first $i$ items, and inside these $i$ prices, there are exactly $C_j$ many of them are $p^{(j)}$ and $\Pr_{i_1,i_2}$ which is the probability that the item, which has the largest gap between its value and price, has value $v^{i_1}$ and price $p^{i_2}$ is in $[\widehat{\Pr}_{i_1,i_2},\widehat{\Pr}_{i_1,i_2}+1/n^3]$. But in each step, we can not store these probabilities accurately since that will require the size of the table to be exponentially big, we will round every probability to an integer multiple of $1/n^3$ which is at most $1/n^3$ away from it in every step. 

\vspace{-8pt} \paragraph{Running Time and Correctness.} Next we bound the algorithm's running time and revenue.

\begin{lemma} \label{lem:dynamic programming revenue}
    Given an instance of {\sc RestrictedPrice}, where the value distributions are supported on a discrete set ${\cal S}$ of cardinality $k_1$ and the prices are restricted to a discrete set ${\cal P}$ of cardinality $k_2$, the algorithm described in this section produces a price vector with expected revenue at least \yangnote{$$OPT -\epsilon\cdot\left({2 \over (nr)^2}+ {16 \over n^{2}} \right)\cdot \min\{ {\cal P} \},$$}
    where $OPT$ is the optimal expected revenue, $\min\{{\cal P}\}$ is the lowest element of $\cal P$, and $r$ is the ratio of the largest to the smallest element of ${\cal P}$.
%    where $\widehat{OPT}$ is the optimal expected revenue for value distributions $\{\hat{F}_i\}_i$ achieved by any price vector in $\left\{p^{(1)},\ldots,p^{(k_2)}\right\}^n$.
\end{lemma}

\begin{lemma}
    The running time of the algorithm is  polynomial in the size of the input and \yangnote{$(\frac{nrk_{1}k_{2}}{\epsilon})^{O\left( k_1 k_2\right)}$}. 
    %$m^{O(k_1k_2)}=m^{O\left({(\log r)^{2}\over\delta^4 }\right)}%
    %$(nr)^{O\left({\log^2 r\over \delta^4 }\right)}$. 
    \label{lem:running time}
\end{lemma}
The proofs of these lemmas are given in Section~\ref{sec:algorithm analysis}. Intuitively, if we did not perform any rounding of distributions, our algorithm would have been  {\em exact}, outputting an optimal price vector in $\{p^{(1)},\ldots,p^{(k_2)}\}^n$. What we show is that the roundings performed at the steps of the dynamic program are fine enough that do not become detrimental to the revenue. To show this, we use the probabilistic concepts of {total variation distance} and {coupling of random variables}, invoking the coupling lemma and the optimal coupling theorem after each step of the algorithm.~(See Lemma~\ref{lem:closeness} in Appendix~\ref{sec:correctness of DP}.) This way, we show that the rounded (winning-value,winning-price) distributions maintained by the algorithm for each price vector are close in total variation distance to the corresponding exact distributions arising from these price vectors, culminating in Lemma~\ref{lem:dynamic programming revenue}.

\notshow{Using Lemmas~\ref{lem:dynamic programming revenue} and~\ref{lem:running time} and our work in the later sections, we obtain our main algorithmic results in this paper (Theorems~\ref{thm:ptas mhr},~\ref{thm:quasi ptas regular},~\ref{thm:general algorithm}, and~\ref{thm:additive ptas}). See Section~\ref{sec:app overall ptas} for the proof of these theorems.}

%\vspace{-10pt}\section{Distributions of Bounded Support} \label{sec:balanced range}


==> regular_old.tex <==
\section{Extreme Values of Regular Distributions}\label{sec:regular}


Our goal is to reduce the problem of finding a near-optimal pricing for a collection of  independent (but not necessarily identical) \textsl{regular} value distributions to the problem of finding a near-optimal pricing for a collection of independent distributions, which are supported on a common finite interval $[u_{min}, u_{max}]$, where $u_{max}/u_{min} \le 16\epsilon^{4}n^8$, where $n$ is the number of distributions, $\epsilon$ is a constant in $(0,1)$. Notice that our bound on the ratio $u_{max}/u_{min}$ does not depend on the distributions at hand, but just their number. Notice also that the input distributions may be supported on $[0,+\infty)$, so it is a priori not clear if we can truncate these distributions to a finite set, not to mention a polynomially-balanced set. 

The following theorem characterize the extreme value of a collection of regular distributions.

\begin{theorem}\label{thm:regextremevalue}
Let $\{x_{i}\}_{i\in[m]}$ be a collection of regular random variables, and $X=\max_{i} x_{i}$. For any integer $n\geq m$, any constant $\epsilon\in (0,1)$, there exists an $\alpha$, such that the followings are true:
\begin{itemize}
\item $\Pr[x_{i}\geq 2\alpha/\epsilon ]\leq \epsilon/n^{3}$ for all $i\in[m]$;
 \item $\alpha/n^{3}\leq c\cdot \max_{z} (z\cdot \Pr[X\geq z])$, for an absolute constant value $c$;
 \item If $t\geq {2n^{2}\alpha\over \epsilon^{2}}$ and $t_{1},\ldots, t_{m}$, s.t. $\forall i\in[m]$, $t_{i}\geq t$, then the following is true.
$$\sum_{i=1}^{m} t_{i} \Pr[x_{i}\geq t_{i}]\leq (t-2\alpha/\epsilon)\Pr[X \geq t]+O\Big{(}{\epsilon\cdot(2\alpha/\epsilon\cdot\max_{i} \Pr[x_{i}\geq 2\alpha/\epsilon])\over n}\Big{)}.$$
\end{itemize}
\end{theorem}

With this theorem, we can argue that if we restrict our prices to be in $[.,2n^{2}\alpha/\epsilon^{2}]$, the optimal revenue for $\{v_{i}\}$ only decreases for $O(\epsilon \cdot\mathcal{R}_{OPT}/n).$

\begin{theorem}\label{thm:regrestrictprice}
    Let $\mathcal{V}=\{v_{i}\}_{i\in[n]}$ be a collection of independent regular value distributions, $\epsilon$ be a constant in $(0,1)$. For any price vector $P$, we can construct a new price vector $\hat{P}\in [\epsilon\alpha/n^{4},2n^{2}\alpha/\epsilon^{2}]^{n}$, such that $\mathcal{R}_{\hat{P}}\geq \mathcal{R}_{P}-O({\epsilon\cdot\mathcal{R}_{OPT}\over n})$.
\end{theorem}
\begin{proof}
	We first construct a price vector $P'\in[0,2n^{2}\alpha/\epsilon^{2}]^{n}$ based on $P$, such that the revenue $\mathcal{P'}$ is at most $O({\epsilon\cdot\mathcal{R}_{OPT}\over n})$ less than $\mathcal{P}$. Let $S=\{i\ \vline\ p_{i}>2n^{2}\alpha/\epsilon^{2}\}$, for any $i\in S$, $p'_{i}={2(n^{2}/\epsilon-1)\alpha\over \epsilon}$, if $i\notin S$, $p'_{i}=p_{i}$.
	
	Let us assume $|S|=m$ and $S=\{a(i)\ \vline\ i\in[m]\}$. Let $x_{i}=v_{a(i)}$. %According to Lemma~\ref{lem:reglittlegain}, $\beta\Pr[v_{i}\geq \beta]\leq {n^{3}\over n^{3}-1} \alpha\Pr[v_{i}\geq \alpha]$ for all $i\in[n]$. Thus, $\Pr[v_{i}\geq \beta]\leq \epsilon/n^{3}$. 
	Now, let $t={2n^{2}\alpha\over \epsilon^{2}}$ and $t_{i} = p_{a(i)}$. Then the contribution to revenue from items in $S$ is upper bounded by $\sum_{i=1}^{m} t_{i} \Pr[x_{i}\geq t_{i}]$. By Theorem~\ref{thm:regextremevalue}, we know it is smaller than $(t-2\alpha/\epsilon)\Pr[X \geq t]+O\Big{(}{\epsilon\cdot(2\alpha/\epsilon\cdot\max_{i} \Pr[x_{i}\geq 2\alpha/\epsilon])\over n}\Big{)}$.
	
	On the other hand, when $\max_{i\in S}\{v_{i}\}=\max_{i} \{x_{i}\}=X\geq t$, the largest gap for items in $S$ is already $2\alpha/\epsilon$. If this item is not the winner, then some item not in $S$ has a larger gap. For this to happen, the value for this item has to be higher than $2\alpha/\epsilon$. However, the probability for any of the items not in $S$ to has value greater than $2\alpha/\epsilon$ is smaller than $n\cdot \epsilon/n^{3}=\epsilon/n^{2}$. Thus, when$X\geq t$, with probability $1-\epsilon/n^{2}$, the winner in $S$ is the actual winner. So when the price vector is $P'$, the revenue from items in $S$ is lower bounded by $(t-2\alpha/\epsilon)\Pr[X \geq t](1-\epsilon/n^{2})$. Obviously, $(t-2\alpha/\epsilon)\Pr[X\geq t]\leq t\Pr[X\geq t] \leq \mathcal{R}_{OPT}$, since we can set every $p_{i}=t$ for all $i\in S$ and all other $p_{i}=+\infty$. Similarly, we can argue that $2\alpha/\epsilon\cdot\max_{i} \Pr[x_{i}\geq 2\alpha/\epsilon]\leq \mathcal{R}_{OPT}$. So we know $$(t-2\alpha/\epsilon)\Pr[X \geq t](1-\epsilon/n^{2})+O({\epsilon\mathcal{R}_{OPT}\over n})\geq \sum_{i=1}^{m} t_{i} \Pr[x_{i}\geq t_{i}].$$ 
	
	Morover, according to Lemma~\ref{lem:trunclow}, which states that we can set prices below $\epsilon\alpha/n^4$ to $\epsilon\alpha/n^4$ and only lose $\epsilon\alpha/n^4\leq {c\epsilon\over n}\cdot \max_{z} (z\cdot \Pr[X\geq z])\leq c\epsilon\mathcal{R}_{OPT}/n$.
	 We can define $\hat{P}$ to be the price vector that if $p'_{i}\leq \epsilon\alpha/n^{4}$, $\hat{p}_{i} = \epsilon\alpha/n^{4}$, otherwise, $\hat{p}_{i}=p'_{i}$. Now we know if we restrict the prices to be in $[\epsilon\alpha/n^4, 2n^2\alpha/\epsilon^{2}]$,the revenue decreases for at most $O({\epsilon\mathcal{R}_{OPT}\over n})$
\end{proof}
{\color{red} I put the proof here just to make sure I basically only use the extreme value theorem plus some other trivial arguments to show the price can be restricted....}

Thus, we have reduce the problem of finding a near-optimal price vector to the problem of finding a near-optimal price vector in the set $[\epsilon\alpha/n^4, 2n^2\alpha/\epsilon^{2}]^{n}$.

For the restricted prices, we can create another collection of bounded the support independent random variables $\tilde{\mathcal{V}}=\{\tilde{v}_i\}_{i\in[n]}$, such that the revenue for the original value distribution and revenue for the bounded value distribution under any price vector in $[\epsilon\alpha/n^4, 2n^2\alpha/\epsilon^{2}]$ are at most  ${\epsilon\mathcal{R}_{OPT}(\mathcal{V})\over c_{1} n}$ different. 

\begin{theorem}\label{thm:regbounding}
   Given a collection of independent regular random variables $\mathcal{V}=\{v_i\}_{i\in[n]}$, for any $\epsilon\in(0,1)$, let us define a new collection of random variables $\tilde{\mathcal{V}}=\{\tilde{v}_i\}_{i\in[n]}$ via the following coupling:  for all $i\in [n]$, set  $\tilde{v}_i={\epsilon\alpha\over 4n^4}$ if $v_i < {\epsilon\alpha\over 2n^4}$, set $\tilde{v}_i=4n^{4}\alpha/\epsilon^{3}$ if $v_i\ge 4n^{4}\alpha/\epsilon^{3}$, and set $\tilde{v}_i=v_i$ otherwise. Then, for any price vector $P\in[\epsilon\alpha/n^{4},2n^{2}\alpha/\epsilon^{2}]^{n}$, $|\mathcal{R}_{P}(\mathcal{V})-{\mathcal{R}}_{P}(\tilde{\mathcal{V}})|\leq {\epsilon\mathcal{R}_{OPT}(\mathcal{V})\over c_{1} n}$.% where $\mathcal{R}_P$ and $\mathcal{R}}_P$ are respectively the revenues of seller when the buyer's values are distributed as $\{v_i\}_{i\in[n]}$ and as $\{\hat{v}_i\}_{i\in[n]}$.
\end{theorem}

This theorem shows that we can reduce the problem of finding a near-optimal price vector in the set $[\epsilon\alpha/n^4, 2n^2\alpha/\epsilon^{2}]^{n}$ for the original value distributions to the problem of finding a near-optimal price vector in the set $[\epsilon\alpha/n^4, 2n^2\alpha/\epsilon^{2}]^{n}$ for the bounded value distributions.  

\begin{theorem}\label{thm:regboundedrestrictprice}
Given a collection of independent regular random variables $\mathcal{V}=\{v_i\}_{i\in[n]}$, for any $\epsilon\in(0,1)$, let us define a new collection of random variables $\tilde{\mathcal{V}}=\{\tilde{v}_i\}_{i\in[n]}$ via the following coupling:  for all $i\in [n]$, set  $\tilde{v}_i={\epsilon\alpha\over 4n^4}$ if $v_i < {\epsilon\alpha\over 2n^4}$, set $\tilde{v}_i=4n^{4}\alpha/\epsilon^{3}$ if $v_i\ge 4n^{4}\alpha/\epsilon^{3}$, and set $\tilde{v}_i=v_i$ otherwise. For any price vector $P$, we can construct a new price vector $\hat{P}\in [\epsilon\alpha/n^{4},2n^{2}\alpha/\epsilon^{2}]^{n}$, such that $\mathcal{R}_{\hat{P}}(\tilde{\mathcal{V}})\geq \mathcal{R}_{P}(\tilde{\mathcal{V}})-O({\epsilon\cdot\mathcal{R}_{OPT}(\tilde{\mathcal{V}})\over n})$
\end{theorem}
The proof is essentially the same as the proof for Theorem~\ref{thm:regrestrictprice}. This theorem show taht we can reduce the problem of finding a near-optimal price vector in the set $[\epsilon\alpha/n^4, 2n^2\alpha/\epsilon^{2}]^{n}$ for the bounded value distributions to the problem of finding a near-optimal price vector for the bounded value distribution.

Combining Theorem~\ref{thm:regrestrictprice},~\ref{thm:regbounding} and~\ref{thm:regboundedrestrictprice}, we can reduce the problem of finding a near-optimal price vector for the original value distributions to the problem of finding a near-optimal price vector for the bounded value distributions. Our reduction is specified by the following theorem.

\begin{theorem}[Reduction from Regular to $Poly(n)$-Balanced Distributions]\label{thm:regreduction}
Let $\mathcal{V}=\{v_i\}_{i\in[n]}$ be a collection of mutually independent \textsl{regular} random variables. For any constant $\epsilon\in(0,1)$, there is a reduction from {\scshape Price}$(\mathcal{V},\epsilon)$ to {\scshape Price}$(\tilde{\mathcal{V}},\epsilon-\Theta(\epsilon/n))$, where $\tilde{\mathcal{V}}=\{\tilde{v}_i\}_{i\in [n]}$ is a collection of mutually independent random variables that are supported on $[{\epsilon\alpha\over 4n^{4}}, {4n^{4}\alpha\over \epsilon^{3}}]$, for some $\alpha=\alpha({\cal V})>0$.
%\item $\alpha$ is defined in Definition~\ref{def:regalpha}.

Moreover, we can compute $\alpha$ in $O(n)$ time, and compute the distributions of variables $\{\tilde{v}_{i}\}_{i\in[n]}$ in time polynomial in $n$, if we have the distributions of the variables $\{v_{i}\}_{i\in[n]}$ explicitly. If we have oracle access to the distributions of the variables $\{v_{i}\}_{i\in[n]}$, we can compute $\alpha$ in time polynomial in $n$ and the desired precision, and construct an oracle for the distributions of the variables $\{\tilde{v}_{i}\}_{i\in[n]}$, running in time polynomial in $n$ and $1/\epsilon$, the input to the oracle and the desired precision. When we have a solution for {\scshape Price}$(\tilde{\mathcal{V}},\epsilon-\Theta(1/n))$, we can construct a solution for {\scshape Price}$(\mathcal{V},\epsilon)$ in time polynomial in $n$ and $1/\epsilon$.
\end{theorem}


Our theorem is based on the following extreme value theorem for regular distributions.

\begin{theorem}
Given a collection of independent regular distributions $\{F_i\}_{i \in [n]}$, there exists an interval $[{\alpha\over 2n^{4}}, 2n^{4}\alpha]$ such that
\end{theorem}

\paragraph{Proof Ideas.} More precisely, we will first compute a number $\alpha$ depending on the value distributions, which can be viewed as the ``center'' of the common interval. The computation takes time linear in $n$. Then, we can efficiently construct a collection of random variables $\tilde{\mathcal{V}}=\{\tilde{v}_{i}\}_{i\in[n]}$ based on $\mathcal{V}=\{v_{i}\}_{i\in[n]}$, such that the following properties are satisfied.
\begin{enumerate}
\item $\forall i$ $\tilde{v}_{i}$ is supported on $[\alpha/f_{1}(n), f_{2}(n)\cdot\alpha]$ for fixed polynomial functions $f_{1}(\cdot)$ and $f_{2}(\cdot)$. The construction is detailed in Lemma~\ref{lem:regboundedtrunchigh} of Appendix~\ref{sec:regrestrictpricebounded}.
\item For any price vector $P$, we can convert it to a new price vector $P'\in [\alpha/f_{3}(n), f_{4}(n)\cdot\alpha]^{n}$ efficiently, where $f_{3}(\cdot)$, $f_{4}(\cdot)$ are fixed polynomial functions, such that the seller's revenue under price $P'$ is at most $O(\mathcal{R}_{OPT}/n)$ less than under price $P$, no matter which the buyers' value distributions are, $\mathcal{V}$ or $\tilde{\mathcal{V}}$. We postpone the proofs to Appendix~\ref{sec:regrestrictprice} and~\ref{sec:regrestrictpricebounded}.
\item For any price vector $P'\in [\alpha/f_{3}(n), f_{4}(n)\cdot\alpha]^{n}$, the seller's revenue when the buyers' values are distributed as $\mathcal{V}$ and the seller's revenue when the buyers' values are distributed as $\tilde{\mathcal{V}}$ are at most $O(\mathcal{R}_{OPT}/n)$ away. All the proofs are postponed to Appendix~\ref{sec:regboundingdistribution}.
\end{enumerate}
 
With the above properties, we can perform our reduction. First, we construct $\tilde{\mathcal{V}}$. Then we find a near-optimal price vector $P$ for value distributions $\tilde{\mathcal{V}}$. Next, we convert it to another price vector $P'\in [\alpha/f_{3}(n), f_{4}(n)\cdot\alpha]^{n}$, then output it as an near-optimal price vector for the original regular value distributions. The reason that $P'$ is the right solution is because we can argue that the optimal revenues for value distributions $\mathcal{V}$ and $\tilde{\mathcal{V}}$ are very close by combining the second and last property, also we know that $P'$ is a near-optimal for $\tilde{\mathcal{V}}$ and it achieves almost the same revenue for $\mathcal{V}$, it has to be that $P'$ is also a near-optimal for $\mathcal{V}$.

To describe the reduction, we first define the ``center'' $\alpha$, unlike in the MHR case, we define the value $\alpha$ here explicitly.
\begin{definition}\label{def:regalpha}
A point is an \textsl{anchoring point}, if  the value of the cumulative distribution at that point is between two a priori known absolute constants $c_{1}$ and $c_{2}$, such that $0 < c_{1} < c_{2} < 1$.  Let $a_{i}$ be the anchoring point of distribution $F_{i}$. Define $\alpha= {n^{3}\over c_{1}}\cdot\max_{i} \Big{[}a_{i}\cdot \big{(}1-F_{i}(a_{i})\big{)}\Big{]}$.
\end{definition}

With $\alpha$, we can formally state our reduction.
\begin{theorem}[Reduction from Regular to $Poly(n)$ Balanced Distributions]\label{thm:regreduction}
Let $\mathcal{V}=\{v_i\}_{i\in[n]}$ be a collection of mutually independent \textsl{regular} random variables. For any constant $\epsilon\in(0,1)$, there is a reduction from {\scshape Price}$(\mathcal{V},\epsilon)$ to {\scshape Price}$(\tilde{\mathcal{V}},\epsilon-\Theta(1/n))$, where 
\begin{itemize}
\item $\tilde{\mathcal{V}}=\{\tilde{v}_i\}_{i\in [n]}$ is a collection of mutually independent random variables that are supported on $[{\alpha\over 2n^{4}}, 2n^{4}\alpha]$;
\item $\alpha$ is defined in Definition~\ref{def:regalpha}.
\end{itemize}
Moreover, we can compute $\alpha$ in $O(n)$ time, and compute the distributions of variables $\{\tilde{v}_{i}\}_{i\in[n]}$ in time polynomial in $n$, if we have the distributions of the variables $\{v_{i}\}_{i\in[n]}$ explicitly. If we have oracle access to the distributions of the variables $\{v_{i}\}_{i\in[n]}$, we can compute $\alpha$ in time polynomial in $n$ and the desired precision, and construct an oracle for the distributions of the variables $\{\tilde{v}_{i}\}_{i\in[n]}$, running in time polynomial in $n$ and $1/\epsilon$, the input to the oracle and the desired precision. When we have a solution for {\scshape Price}$(\tilde{\mathcal{V}},\epsilon-\Theta(1/n))$, we can construct a solution for {\scshape Price}$(\mathcal{V},\epsilon)$ in time polynomial in $n$ and $1/\epsilon$.
\end{theorem}

==> regular_oldest.tex <==
\section{Extreme Values of Regular Distributions}\label{sec:regular}


Our goal is to reduce the problem of finding a near-optimal pricing for a collection of  independent (but not necessarily identical) \textsl{regular} value distributions to the problem of finding a near-optimal pricing for a collection of independent distributions, which are supported on a common finite interval $[u_{min}, u_{max}]$, where $u_{max}/u_{min} \le 4n^8$, where $n$ is the number of distributions. Notice that our bound on the ratio $u_{max}/u_{min}$ does not depend on the distributions at hand, but just their number. Notice also that the input distributions may be supported on $[0,+\infty)$, so it is a priori not clear if we can truncate these distributions to a finite set, not to mention a polynomially-balanced set. 


Our reduction is specified by the following theorem.

\begin{theorem}[Reduction from Regular to $Poly(n)$-Balanced Distributions]\label{thm:regreduction}
Let $\mathcal{V}=\{v_i\}_{i\in[n]}$ be a collection of mutually independent \textsl{regular} random variables. For any constant $\epsilon\in(0,1)$, there is a reduction from {\scshape Price}$(\mathcal{V},\epsilon)$ to {\scshape Price}$(\tilde{\mathcal{V}},\epsilon-\Theta(1/n))$, where $\tilde{\mathcal{V}}=\{\tilde{v}_i\}_{i\in [n]}$ is a collection of mutually independent random variables that are supported on $[{\alpha\over 2n^{4}}, 2n^{4}\alpha]$, for some $\alpha=\alpha({\cal V})>0$.
%\item $\alpha$ is defined in Definition~\ref{def:regalpha}.

Moreover, we can compute $\alpha$ in $O(n)$ time, and compute the distributions of variables $\{\tilde{v}_{i}\}_{i\in[n]}$ in time polynomial in $n$, if we have the distributions of the variables $\{v_{i}\}_{i\in[n]}$ explicitly. If we have oracle access to the distributions of the variables $\{v_{i}\}_{i\in[n]}$, we can compute $\alpha$ in time polynomial in $n$ and the desired precision, and construct an oracle for the distributions of the variables $\{\tilde{v}_{i}\}_{i\in[n]}$, running in time polynomial in $n$ and $1/\epsilon$, the input to the oracle and the desired precision. When we have a solution for {\scshape Price}$(\tilde{\mathcal{V}},\epsilon-\Theta(1/n))$, we can construct a solution for {\scshape Price}$(\mathcal{V},\epsilon)$ in time polynomial in $n$ and $1/\epsilon$.
\end{theorem}


Our theorem is based on the following extreme value theorem for regular distributions.

\begin{theorem}
Given a collection of independent regular distributions $\{F_i\}_{i \in [n]}$, there exists an interval $[{\alpha\over 2n^{4}}, 2n^{4}\alpha]$ such that
\end{theorem}

\paragraph{Proof Ideas.} More precisely, we will first compute a number $\alpha$ depending on the value distributions, which can be viewed as the ``center'' of the common interval. The computation takes time linear in $n$. Then, we can efficiently construct a collection of random variables $\tilde{\mathcal{V}}=\{\tilde{v}_{i}\}_{i\in[n]}$ based on $\mathcal{V}=\{v_{i}\}_{i\in[n]}$, such that the following properties are satisfied.
\begin{enumerate}
\item $\forall i$ $\tilde{v}_{i}$ is supported on $[\alpha/f_{1}(n), f_{2}(n)\cdot\alpha]$ for fixed polynomial functions $f_{1}(\cdot)$ and $f_{2}(\cdot)$. The construction is detailed in Lemma~\ref{lem:regboundedtrunchigh} of Appendix~\ref{sec:regrestrictpricebounded}.
\item For any price vector $P$, we can convert it to a new price vector $P'\in [\alpha/f_{3}(n), f_{4}(n)\cdot\alpha]^{n}$ efficiently, where $f_{3}(\cdot)$, $f_{4}(\cdot)$ are fixed polynomial functions, such that the seller's revenue under price $P'$ is at most $O(\mathcal{R}_{OPT}/n)$ less than under price $P$, no matter which the buyers' value distributions are, $\mathcal{V}$ or $\tilde{\mathcal{V}}$. We postpone the proofs to Appendix~\ref{sec:regrestrictprice} and~\ref{sec:regrestrictpricebounded}.
\item For any price vector $P'\in [\alpha/f_{3}(n), f_{4}(n)\cdot\alpha]^{n}$, the seller's revenue when the buyers' values are distributed as $\mathcal{V}$ and the seller's revenue when the buyers' values are distributed as $\tilde{\mathcal{V}}$ are at most $O(\mathcal{R}_{OPT}/n)$ away. All the proofs are postponed to Appendix~\ref{sec:regboundingdistribution}.
\end{enumerate}
 
With the above properties, we can perform our reduction. First, we construct $\tilde{\mathcal{V}}$. Then we find a near-optimal price vector $P$ for value distributions $\tilde{\mathcal{V}}$. Next, we convert it to another price vector $P'\in [\alpha/f_{3}(n), f_{4}(n)\cdot\alpha]^{n}$, then output it as an near-optimal price vector for the original regular value distributions. The reason that $P'$ is the right solution is because we can argue that the optimal revenues for value distributions $\mathcal{V}$ and $\tilde{\mathcal{V}}$ are very close by combining the second and last property, also we know that $P'$ is a near-optimal for $\tilde{\mathcal{V}}$ and it achieves almost the same revenue for $\mathcal{V}$, it has to be that $P'$ is also a near-optimal for $\mathcal{V}$.

To describe the reduction, we first define the ``center'' $\alpha$, unlike in the MHR case, we define the value $\alpha$ here explicitly.
\begin{definition}\label{def:regalpha}
A point is an \textsl{anchoring point}, if  the value of the cumulative distribution at that point is between two a priori known absolute constants $c_{1}$ and $c_{2}$, such that $0 < c_{1} < c_{2} < 1$.  Let $a_{i}$ be the anchoring point of distribution $F_{i}$. Define $\alpha= {n^{3}\over c_{1}}\cdot\max_{i} \Big{[}a_{i}\cdot \big{(}1-F_{i}(a_{i})\big{)}\Big{]}$.
\end{definition}

With $\alpha$, we can formally state our reduction.
\begin{theorem}[Reduction from Regular to $Poly(n)$ Balanced Distributions]\label{thm:regreduction}
Let $\mathcal{V}=\{v_i\}_{i\in[n]}$ be a collection of mutually independent \textsl{regular} random variables. For any constant $\epsilon\in(0,1)$, there is a reduction from {\scshape Price}$(\mathcal{V},\epsilon)$ to {\scshape Price}$(\tilde{\mathcal{V}},\epsilon-\Theta(1/n))$, where 
\begin{itemize}
\item $\tilde{\mathcal{V}}=\{\tilde{v}_i\}_{i\in [n]}$ is a collection of mutually independent random variables that are supported on $[{\alpha\over 2n^{4}}, 2n^{4}\alpha]$;
\item $\alpha$ is defined in Definition~\ref{def:regalpha}.
\end{itemize}
Moreover, we can compute $\alpha$ in $O(n)$ time, and compute the distributions of variables $\{\tilde{v}_{i}\}_{i\in[n]}$ in time polynomial in $n$, if we have the distributions of the variables $\{v_{i}\}_{i\in[n]}$ explicitly. If we have oracle access to the distributions of the variables $\{v_{i}\}_{i\in[n]}$, we can compute $\alpha$ in time polynomial in $n$ and the desired precision, and construct an oracle for the distributions of the variables $\{\tilde{v}_{i}\}_{i\in[n]}$, running in time polynomial in $n$ and $1/\epsilon$, the input to the oracle and the desired precision. When we have a solution for {\scshape Price}$(\tilde{\mathcal{V}},\epsilon-\Theta(1/n))$, we can construct a solution for {\scshape Price}$(\mathcal{V},\epsilon)$ in time polynomial in $n$ and $1/\epsilon$.
\end{theorem}


